From Textual Columns to Query Plans: A Unified Relational-Semantic Execution Framework for Hybrid Query Processing

Real-world table question answering often involves hybrid schemas in which some query-relevant information is explicit in relational columns, while other attributes, predicates, or join conditions are only implicit in free-form text. Existing systems struggle with this setting: Text-to-SQL methods scale to large and multi-table databases but require fully structured schemas, whereas direct LLM-based methods can interpret textual content but are costly and unreliable when applied to large databases. We present OmniTQA, a unified framework for semi-structured table question answering that treats semantic reasoning as a first-class operation within relational query execution. OmniTQA compiles natural-language questions into directed acyclic graphs of relational and LLM-based semantic operators. This enables ambiguity-aware plan diversification, cost-aware optimization, and dual-engine execution over structured and textual data. Across structured and semi-structured benchmarks, OmniTQA consistently improves performance in hybrid settings, outperforming the strongest baselines by 14 accuracy points on average and by 27 points on the most challenging subset, while maintaining competitive accuracy on fully structured datasets.

==> 1_introduction.tex <==
\section{Introduction}

\begin{figure*}[t]
  \centering
  \includegraphics[scale = 0.55]{figures/toy_example.pdf}
  \vspace{-1.5em}
  \caption{\small Two instances of \textsf{NCAA Soccer} database with distinct schema representations: (left) structured; (right) semi-structured.}
  \vspace{-1em}
  \label{fig:example-figure}
\end{figure*}

%Natural language (NL) interfaces allow users to query databases without writing SQL. 
Recent advances in large language models (LLMs) have significantly improved Text-to-SQL and table question answering systems, making them a key component of modern data access interfaces \cite{ipeirotis2025natural, liu2025survey, zhang2024natural}. These systems achieve strong performance when queries can be mapped to structured schemas and executed using relational operators. However, these approaches rely on a key assumption: all query-relevant information is explicitly represented in structured attributes. In practice, this assumption rarely holds. Many real-world datasets contain \textit{hybrid} schemas where structured attributes coexist with free-form text fields that implicitly
%such as product descriptions or clinical notes. 
%These fields often 
encode entities, predicates, or relational references not materialized as explicit columns. Consequently, answering even simple queries may require extracting latent structure from text before performing relational reasoning.

This mismatch introduces a key challenge for natural language query processing. In fully structured databases, answering a question reduces to  mapping predicates to schema attributes and executing relational operations such as selection, join, and aggregation. In contrast, when relevant information is embedded in textual fields, systems must interleave semantic reasoning (e.g., extracting entities, resolving predicates, performing fuzzy matching) with symbolic relational processing. This requires jointly reasoning over heterogeneous data representations while maintaining efficiency and scalability. The following example illustrates this contrast.

%\vspace{-1em}
\begin{example}\label{ex:1}
\small
Consider the \textsf{NCAA Soccer} database with relations \textsf{College} and \textsf{Tryout}, shown on the left side of Figure~\ref{fig:example-figure}. 
Suppose a user poses a query:
\textit{``What is the tryout ID and the state of the college where a goalie player was successfully accepted?''}

In this structured setting, a Text-to-SQL system can directly map the NL query to a SQL query with a selection operation over the \textsf{Tryout} table followed by a join operation with the \textsf{College} table and a projection operation over the requested attributes.
\end{example}

% \vspace{-1em}
\begin{example}\label{ex:2}
\small
Consider the semi-structured instance of the same database shown on the right side of Figure~\ref{fig:example-figure}. Here, key attributes such as position, decision, and state are embedded within textual descriptions.

Answering the same query now requires several semantic reasoning steps:

(i) identifying tuples in \textsf{Tryout} mentioning both the \textit{goalie} position and a successful admission,
(ii) extracting the college name from the text,
(iii) matching this entity with the \textsf{College} relation, and (iv) extracting the state from the text before producing the final projection.
\end{example}


Existing approaches fall short in this setting. 
Text-to-SQL systems are tightly coupled to explicit schema attributes and cannot operate when predicates or join keys are implicitly encoded in text \cite{zhou2025table}. LLM-based table question answering methods \cite{fanglarge,yu-etal-2025-table} treat tables as serialized text and reason directly over it. While effective for small tables or single relations, these approaches scale poorly to large datasets and multi-table schemas and incur substantial inference cost \cite{zhang2025same}. 
{
  Recent hybrid systems \cite{khoja2025weaver,abhyankar2025h,patel2025semantic,chengbinding} combine relational execution with LLM-based semantic operators to enable more flexible query processing such as semantic filtering and aggregation. However, these approaches typically assume that schema attributes are well-defined and apply semantic operators only to interpret or match values within individual columns.
  They are less suited for scenarios where a single textual field conflates multiple latent attributes and relational references that would otherwise be represented as separate columns.
  In such cases, query-relevant structure is not explicitly materialized and cannot be recovered through schema resolution alone. Instead, the system must reconstruct this structure from entangled textual descriptions prior to applying  relational operations. Enabling this requires a tighter integration of semantic reasoning with query planning and execution. Table~\ref{tab:tqa_comparison} provides a high-level picture of how existing approaches handle key challenges such as long tables, multi-table reasoning, complex queries, and implicit schema.
}

To address these limitations, we introduce Semi-structured Table Question Answering (\Problem), a setting where natural language queries operate over relational databases containing both structured attributes and textual columns. 
{
 In \Problem, predicates, entities, and join attributes may be explicitly represented in the schema, implicitly embedded within textual fields, or not materialized as standalone attributes at all. 
 Solving \Problem therefore requires more than executing queries over existing schema elements. It must identify, extract, align, and compose missing structural signals from unstructured textual fields during query processing.
}
% In \Problem, predicates or join attributes may appear either explicitly in the schema or implicitly within text. 
% \Problem requires systems to not only execute queries, but also dynamically recover structured signals from unstructured data during query processing.


In response, we present \System, a hybrid query processing system for \Problem that treats semantic reasoning as a \textit{first-class query operator} within a relational execution model.  It translates NL queries into executable directed acyclic graphs (DAGs) of atomic operators, where each node corresponds to either a relational or an LLM-based semantic operator.
%(e.g., semantic filtering, entity extraction, or fuzzy joins). 
This atomic operator-centric design enables fine-grained decomposition, tight integration of symbolic and semantic reasoning, and execution plans with explicit semantics.
% This design enables fine-grained decomposition into atomic operators through query-aware data preview, principled cost-based optimization across semantic and relational steps, and execution plans with explicit semantics.
%Concretely, This operator-centric formulation enables tight integration of symbolic and semantic reasoning within a unified execution framework. 
Building on this abstraction, \System performs data-aware planning and cost-efficient execution over hybrid schemas. It incorporates optimization strategies such as relational pruning, operator reordering, and query-aware data reduction to explicitly account for the asymmetry between inexpensive relational operations and costly semantic operators. 
%These techniques significantly reduce the volume of data processed by LLMs, improving both efficiency and scalability. 

% translates NL queries into executable query plans represented as directed acyclic graphs (DAGs) of atomic operators, where each operator corresponds to either a relational computation or an LLM-based semantic operation such as semantic filtering, entity extraction, or fuzzy joins. \nb{Unlike prior approaches that focus primarily on extending relational query languages, OmniTQA emphasizes data-aware planning and execution over hybrid schemas. The system decomposes queries into fine-grained atomic steps, enabling flexible integration of symbolic and semantic reasoning. It further introduces optimization strategies that minimize the cost of semantic operations by leveraging relational pruning, operator reordering, and query-aware data reduction. These techniques reduce the volume of data processed by LLMs, which are more expensive than relational operations. } 

%{\System translates NL queries into executable hybrid query plans represented as directed acyclic graphs (DAGs) of atomic operators executed either by the database engine or an LLM reasoning module. This representation enables principled optimization of hybrid queries. \System extends classical query optimization to the hybrid setting by reasoning about the cost asymmetry between relational operations and semantic inference. In particular, it reorders operators to minimize the amount of data processed by semantic operators, thus reducing inference latency and token consumption.}

To execute these plans efficiently, \System introduces a \textit{dual-engine execution architecture} that dynamically routes operators to either a relational database engine or an LLM-based reasoning module. It further incorporates \textit{operator-aware batching}, partitioning intermediate relations and executing semantic operations in parallel. Together, these mechanisms enable scalable semantic reasoning over large  datasets while respecting LLM context constraints and controlling inference cost. Beyond augmenting structured queries, \System reconstructs latent attributes, predicates, and relationships directly from textual fields during query execution. 
% Table~\ref{tab:tqa_comparison} provides a high-level comparison of how \System and existing approaches handle key challenges such as long tables, multi-table reasoning, complex queries, and implicit schema.

We evaluate \System across a diverse suite of table question answering benchmarks spanning structured, semi-structured, and multi-table settings. Experimental results demonstrate that it consistently outperforms existing symbolic, semantic, and hybrid baselines in both accuracy and cost efficiency, particularly for complex queries involving large tables and multi-relation schemas.


Our main contributions are as follows:

\begin{itemize}[leftmargin=*]
    \item {We introduce Semi-structured Table Question Answering ($\Problem$), a new problem setting where query-relevant may be explicitly represented, embedded in textual fields, or not materialized as standalone schema attributes.}
    
    %We formalize the problem of Semi-structured Table Question Answering ($\Problem$), where query predicates and join attributes may appear within textual database fields.
    
    \item We propose a hybrid query processing framework for \Problem that integrates relational and LLM-based semantic operators within executable DAG-based query plans, enabling unified reasoning over structured and textual data.
    
    \item We develop data-aware planning and optimization techniques that support complex queries over large and multi-relation datasets by minimizing expensive semantic computation via relational pruning, operator reordering, and query-aware data reduction.
    
    %that minimize expensive semantic computation through relational pruning, operator reordering, and query-aware data reduction.

    \item We design a dual-engine execution framework with operator-aware batching strategies for scalable processing of long tables and efficient handling of hybrid workloads.
    %to scale over large relational datasets.
    

    \item We conduct an extensive empirical evaluation across 12 benchmark datasets and 3 LLMs, demonstrating substantial improvements in both accuracy and cost-efficiency over state-of-the-art symbolic, semantic, and hybrid baselines.
\end{itemize}

\newcommand{\cmark}{\ding{51}}
\newcommand{\xmark}{\ding{55}}

\begin{table}[t]
\centering
\scriptsize
\caption{Comparison of existing TQA approaches vs. \System. \xmark{} denotes settings that are not natively supported, although limited or indirect handling may still be feasible.}
\label{tab:tqa_comparison}
\vspace{-1em}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{@{} l|c|c|c|c @{}}
\toprule
\textbf{Challenge} & \textbf{NL2SQL} & \textbf{Direct-LLM} & \textbf{Hybrid} & \textbf{\System} \\ 
\midrule
Long tables       & \cmark  & \xmark  & \xmark  & \cmark \\ \hline
Multi-table       & \cmark  & \cmark  & \xmark  & \cmark \\ \hline
Complex queries   & \cmark  & \xmark  & \xmark  & \cmark \\ \hline
Textual columns   & \xmark  & \cmark  & \cmark  & \cmark \\ \hline
Implicit schema   & \xmark  & \cmark  & \xmark  & \cmark \\ 
\bottomrule
\end{tabular}
\end{table}

==> 2_preliminary.tex <==
\section{Preliminaries}\label{sec:preliminary}

\subsection{Data Model}
Let $\Schema=\{\Relation_1,\dots,\Relation_n\}$ be a relational schema where each relation $\Relation_i$ is defined over attributes $\AttrRel=\{A_{i,1},\dots,A_{i,m_i}\}$. We denote the global attribute set as $\Attr=\bigcup_i \AttrRel$. To model heterogeneous data, we partition attributes into structured and unstructured subsets, $\Attr=\AttrS \cup \AttrU$ with $\AttrS \cap \AttrU=\emptyset$. Structured attributes $\AttrS$ admit standard relational operations (e.g., numeric, categorical, temporal), while unstructured attributes $\AttrU$ contain free-form textual content. A relation may therefore contain attributes from both subsets, forming a hybrid schema. A database instance over $\Schema$ is denoted by $\Database=\{\Instance_1,\dots,\Instance_n\}$, where each $\Instance_i$ is a finite set of tuples conforming to $\Relation_i$.
% Let $\Schema = \{\Relation_1, \dots, \Relation_n\}$ be a relational schema.
% Each relation $\Relation_i \in \Schema$ is defined over a set of attributes
% $\AttrRel = \{A_{i,1}, \dots, A_{i,m_i}\}$.
% We define the global attribute universe as
% $\Attr = \bigcup_{i=1}^n \AttrRel$.
% To capture heterogeneous data types, we conceptually partition $\Attr$ into two disjoint subsets ($\AttrS \cup \AttrU = \Attr, \AttrS \cap \AttrU = \emptyset$), where $\AttrS$ denotes structured attributes whose domains admit standard relational operations (e.g., numeric, categorical, temporal), and $\AttrU$ represents unstructured attributes containing free-form textual content.
% A relation schema $\Relation_i$ may contain attributes from both $\AttrS$ and $\AttrU$, resulting in hybrid schemas.

% A database instance over $\Schema$ is denoted by $\Database = \Instances$, where each $\Instance_i$ is a finite set of tuples conforming to schema $\Relation_i$.
% Each tuple $\Tuple \in \Instance_i$ is represented as a vector $\Tuple = (\Value_{i,1}, \dots, \Value_{i,m_i}),$
% where $\Value_{i,j} \in \Domain(A_{i,j})$.
% If $A_{i,j} \in \AttrS$, then $\Value_{i,j}$ is a structured value;
% if $A_{i,j} \in \AttrU$, then $\Value_{i,j}$ is free-form textual content.

\subsection{Table Question Answering}
We first review the classical \textsf{TQA} setting, where database schemas contain only structured attributes ($\Attr=\AttrS$). Query answering therefore reduces to executing relational operations over the data.

% We start by reviewing the well-known \textsf{TQA} problem. In \textsf{TQA}, the database schema $\Schema$ consists exclusively of structured
% attributes (i.e., $\Attr = \AttrS$).
% Thus, every relation schema $\Relation_i \in \Schema$ contains only attributes
% whose domains admit standard relational operations. The problem is defined as follows:

\begin{definition}[Table Question Answering ---\textsf{TQA}]    
Let $\Schema$ be a relational schema such that $\Attr = \AttrS$ 
(i.e., $\AttrU = \emptyset$).
Given a natural language question $\Question$ and a database instance 
$\Database$ defined over $\Schema$, the \textsf{TQA} problem concerns 
computing an answer $\Answer$ such that
\[
\Model : (\Question, \Database) \rightarrow \Answer,
\]
where $\Answer$ is a set of tuples, a projection thereof, or an aggregate value
derived solely through relational operations over $\AttrS$.
\end{definition}

In this setting, \textsf{TQA}  reduces to constructing and executing a query plan composed of classical operators (e.g., $\Select$, $\Project$, $\Join$, $\Aggregate$).

% -- nikita: commenting out in the interest of space
% \begin{table}[t]
% \footnotesize
% \centering
% \caption{Table of Notations}
% \vspace{-1em}
% \label{tab:notation}
% \begin{tabular}{l|l}
% \toprule
% \textbf{Notation} & \textbf{Definition} \\
% \midrule
% $\Schema$ & Database schema \\\hline
% $\Relation_i$ & Schema of the $i$-th relation \\\hline
% $\AttrRel$ & Set of attributes of relation $\Relation_i$ \\\hline
% $\Attr$ & Global set of all attributes in $\Schema$ \\\hline
% $\AttrS$ & Structured attributes \\\hline
% $\AttrU$ & Unstructured attributes \\\hline
% $\Database$ & Database instance over $\Schema$ \\\hline
% $R_i$ & Instance (set of tuples) of relation $\Relation_i$ \\\hline
% $\Tuple$ & A single tuple in a relation $R_i$ \\\hline
% $\Value_{i,j}$ & Value of attribute $A_{i,j}$ in tuple $\Tuple$ \\\hline
% $\Domain(A)$ & Domain of attribute $A$ \\\hline
% $\Question$ & Natural language question \\\hline
% $\Answer$ & Answer to the question $\Question$ \\
% \bottomrule
% \end{tabular}
% \vspace{-1em}
% \end{table}

\subsection{Problem Formulation}

We now formally define our problem of interest.
%With the necessary terms and notations defined, we now formally define our problem of interest:
\begin{definition}[Semi-structured Table Question Answering --- $\Problem$]
Let $\Schema$ be a hybrid relational schema over $\Attr = \AttrS \cup \AttrU$ attributes.  
Given a natural language question $\Question$ and a database instance $\Database$ defined over $\Schema$, the goal of $\Problem$ is to compute an answer $\Answer$ that satisfies the information need expressed in $\Question$.
% Formally, $\Problem$ seeks to compute a function:
\[
\Model : (\Question, \Database) \rightarrow \Answer,
\] 
where $\Answer$ belongs to a well-defined answer domain (e.g., a set of tuples, a projection thereof, or an aggregate value derived from $\Database$).  

\end{definition}

Unlike traditional Text-to-SQL, which assumes reasoning exclusively over structured attributes $\AttrS$, $\Problem$ requires hybrid execution across both attribute types:

\begin{enumerate}[leftmargin=*]
    \item \textbf{Symbolic Reasoning:}
    applying relational operators (e.g., $\Select$, $\Project$, $\Join$, $\Aggregate$) over attributes in $\AttrS$.

    \item \textbf{Semantic Reasoning:}
    performing semantic retrieval, matching, information extraction, semantic joins or aggregates over textual content in attributes in $\AttrU$ to derive predicates, relevance scores, or extracted structured signals.

    \item \textbf{Joint Processing:}
    integrating symbolic and semantic reasoning steps within a unified execution pipeline.
    % Integrating symbolic and semantic reasoning steps within a unified execution process, where signals derived from $\AttrU$ may influence relational predicates, join conditions, or aggregation scopes.
\end{enumerate}

The core challenge of $\Problem$ lies in the principled integration of relational query processing with semantic text understanding, enabling efficient end-to-end reasoning over hybrid schemas.



==> 3_system_overview.tex <==
\section{System Overview}\label{sec:overview}

\begin{figure*}[h]
  \centering
  \includegraphics[width=\textwidth]{figures/architecture.pdf}
  \vspace{-2.0em}
  \caption{End-to-end overview of the \System framework.}
  \vspace{-1em}
\label{fig:system_architecture}
\end{figure*}

% \begin{figure*}[t]
%   \centering
%   \includegraphics[width=\textwidth]{figures/running_example.pdf}
%   \vspace{-2.0em}
%   \caption{Running example of a \textsf{UEFA Soccer} database.}
%   \vspace{-1em}
% \label{fig:running_example}
% \end{figure*}

% \begin{figure*}[t]
%   \centering
%   \includegraphics[width=\textwidth]{figures/k-plans.pdf}
%   \vspace{-2.5em}
%   \caption{Three initial query plans and their corresponding optimized versions for running example~\ref{ex:running_example_1}.}
%   \vspace{-1em}
% \label{fig:running_example_decomposition}
% \end{figure*}

{The \Problem setting requires integrating two fundamentally different forms of computation: scalable relational query processing and semantic interpretation of textual attributes. Relational operators provide efficient data filtering and joining, while LLM-based reasoning enables extraction and interpretation of information embedded in text. A practical system must therefore combine these capabilities while minimizing the cost of expensive semantic reasoning. To address this challenge, we design \System, a hybrid query processing system that unifies relational execution and semantic operators within a single query planning and execution framework.
}

{Figure ~\ref{fig:system_architecture} shows the overall architecture of \System. Given a natural language query and a database instance, it produces a structured result through three stages:}

\begin{enumerate}[leftmargin=*]

\item \textbf{Pre-processing}, which prepares schema and data context for query planning.

\item \textbf{Planning and Optimization}, which translates the query into an executable hybrid plan and applies cost-aware optimization.

\item \textbf{Execution}, which evaluates the plan using both relational and semantic operators.
\end{enumerate}

% \begin{enumerate}[leftmargin=*]
% \item \nb{\textbf{Hybrid Operator Model.} Query processing should seamlessly combine symbolic relational operators with semantic operators that interpret textual attributes. Treating semantic reasoning tasks as first-class operators enables them to be integrated directly within relational query plans.}

% \item \nb{\textbf{Structured Query Decomposition.} Rather than relying on monolithic LLM reasoning over entire tables, queries should be decomposed into structured execution plans composed of atomic operators. This decomposition improves interpretability, and enables systematic optimization of hybrid query plans.}

% \item \nb{\textbf{Cost-Aware Hybrid Optimization.} Since semantic reasoning is significantly more expensive than symbolic computation, query plans should minimize the amount of data processed by semantic operators through relational pruning and operator reordering.}

% \item \nb{\textbf{Scalable Hybrid Execution.} Hybrid query execution must scale to large relational datasets despite LLM context limitations, requiring strategies that partition intermediate relations and exploit parallelism.}
% \end{enumerate}

% \nb{Together, these principles enable the integration of relational query processing with LLM-based semantic reasoning in a scalable and principled manner. We illustrate the overall architecture of \System in Figure ~\ref{fig:system_architecture}.}

% \System processes user queries through a multi-phase pipeline, illustrated in Figure~\ref{fig:system_architecture}. 

\stitle{Pre-processing}
{The preprocessing stage prepares the database context used during planning. It resolves structural inconsistencies, eliminates irrelevant tables and attributes, augments the schema with light-weight data profiles and constructs query-aware data preview consisting of semantically relevant rows and representative samples. These artifacts provide the planner with grounded information about the schema and underlying data distribution.}

% The preprocessing stage prepares the database context for query planning, especially by refining the database schema and pruning irrelevant context. 
% % The system begins with a preprocessing phase designed to refine the database schema and prune irrelevant context. 
% This phase serves four primary objectives:
% \begin{itemize}[leftmargin=*]
%     \item Resolving structural inconsistencies and formatting anomalies to prevent downstream execution errors.
%     \item Reducing token overhead through high-recall pruning strategies that eliminate irrelevant tables and attributes while preserving the necessary context for planning.
%     \item Enriching the schema with data profiles, including attribute types, statistical summaries, and relational constraints (e.g., primary and foreign keys) to improve mapping accuracy.
%     \item Enhancing the planner's context by providing a hybrid sample of the database, consisting of rows semantically similar to the user query alongside a representative set of random rows.
% \end{itemize}

\stitle{Planning and Optimization} 
In the planning stage, \System decomposes the NL query into a DAG of atomic operators. Each operator corresponds to a relational operation executed by the database engine or a semantic operation executed by an LLM-based  module.  
This representation enables unified symbolic and semantic reasoning within a single interpretable execution plan. Atomic steps maximize delegation to the efficient relational engine and reduce LLM non-determinism by constraining the output space. To address schema ambiguity in tables and LLM variance, \System generates multiple candidate plans under a fixed computation budget. Given the high cost of semantic operations, it applies cost-aware optimization to minimize their usage. It pushes relational filters and projections toward data sources to prune irrelevant tuples before invoking semantic reasoning.

% skipping details to later section.
%In the planning stage, OmniTQA translates the natural language query into a structured execution plan. Rather than generating a single SQL query, the system decomposes the query into a directed acyclic graph (DAG) of atomic operations. 
% This planner is \textit{schema-and-data-aware}, conditioning its generation on table metadata, attribute types, and available operator signatures. Each node in this DAG corresponds to a predefined operator drawn from a finite universe of symbolic and semantic operators.
 
% This approach serves three critical functions: 
% (i) It mitigates the inherent non-determinism of LLM planners by enforcing a restricted output space.
% (ii) It allows the system to leverage a finite set of symbolic and semantic operators to transform each step into a fully structured execution instruction. \nima{Add: using SQL more, less cost.}
% (iii) It provides a transparent lineage, allowing users to trace the provenance of intermediate results through interpretable steps.

% To address linguistic ambiguity and LLM variance, \System can generate multiple candidate plans under a specified computational budget. This multi-plan strategy enables the exploration of alternative semantic interpretations—such as under-specified predicates or implicit joins—and reduces downstream execution error through repeated sampling.

% Once candidate plans are generated, they undergo a systematic optimization phase designed to minimize computational latency and monetary cost while preserving semantic equivalence. Our optimizer leverages the cost asymmetry between inexpensive symbolic computation and expensive semantic reasoning:
% \begin{itemize}[leftmargin=*]
%     \item We apply classical relational heuristics by moving symbolic selection ($\sigma$) and projection ($\pi$) operators as close to the base relations as possible. By pruning irrelevant tuples and attributes early in the DAG, we minimize the cardinality of intermediate results passed to subsequent stages.
%     \item Semantic operators are deliberately deferred until the latest possible stage in the plan. By ensuring these operators only execute on pre-filtered, minimized datasets, we significantly reduce both financial overhead and total execution time.
%     \item Joins are handled based on their predicate types. For symbolic joins, we employ cost-based reordering to prioritize relations with high-selectivity predicates. For hybrid joins involving semantic conditions (e.g., similarity joins), the system first evaluates symbolic components to restrict the candidate space. Semantic reasoning is then invoked only on the reduced set of tuple pairs. In cases where a join depends solely on semantic predicates, we utilize lightweight pre-filtering (e.g., lexical overlap) to prune the candidate space before invoking the LLM. 
% \end{itemize}

\stitle{Execution} {The execution stage evaluates optimized plans using a dual-engine architecture, with multiple plans evaluated in parallel. Relational operators are executed as SQL queries, while semantic operators are handled by the LLM-based module. To scale to large datasets, semantic operations are batched over partitioned intermediate results and executed in parallel.}
%To ensure scalability when processing large relations, semantic operators are executed using operator-aware batching strategies that partition intermediate relations into manageable subsets and process them in parallel.}

%In the third phase, each generated and optimized query plan is executed, with multiple plans evaluated in parallel. Within a given plan, execution follows the structure of its DAG. Since each atomic step depends only on the outputs of its parent nodes, we exploit this partial ordering to parallelize execution across independent nodes at the same level of the DAG. This level-wise parallelization reduces end-to-end latency while preserving correctness under the plan’s dependency constraints.
% As described earlier, each atomic step corresponds to an operator drawn from a predefined universe of symbolic and semantic operators. Execution is therefore operator-driven: depending on the operator type, each step is routed to the appropriate execution engine.

% For symbolic operators, the structured step specification is forwarded to a Text-to-SQL agent, which translates the instruction into an executable SQL query. The resulting SQL statement is executed directly on the underlying database engine, producing either an intermediate relation or a final result table.

% For semantic operators, the step specification and its associated input tables are passed to an LLM-based executor. As previously mentioned, since LLMs operate under context-length and cost constraints, naive execution over large intermediate tables would be infeasible. To address this challenge, our LLM-based executor supports batched execution: the input relation is partitioned into manageable subsets, and the semantic operation is applied incrementally across batches. This batching mechanism ensures scalability while preserving semantic consistency across partitions. Upon completion of semantic reasoning, the resulting outputs are materialized back into the database as structured tables using SQL operations. 

\stitle{Consolidation} After executing all candidate plans, \System selects the most appropriate result using a set of practical plan-selection strategies, or delegates this decision to a human expert. The following sections describe each stage in detail.

{In summary, \System is guided by three key design principles: (i) treating semantic reasoning as a first-class operator to enable unified planning, (ii) minimizing expensive semantic computation through data-aware optimization, and (iii) leveraging plan diversification to mitigate schema ambiguity in tables. These principles jointly enable robust and scalable query processing over semi-structured data.}
% \vspace{-0.5em}
% In Sections~\ref{sec:preprocessing},~\ref{sec:planning}, and~\ref{sec:execution}, we present the technical contributions and implementation details of each phase.
 
% We will further use the following running example to illustrate them.

% The following sections describe each stage in detail.
% \begin{runningexample}\label{ex:planning}
% Consider the \textsf{UEFA Soccer} database shown in Figure~\ref{fig:planning}. 
% %Suppose a user submits the query: 
% Let the query of interest be:
% \textit{``Did the best player of year 2021 win the UCL championship?''} 

% Given the database and the NL query, \System executes the following steps:
% \begin{itemize}[leftmargin=*]
%     \item \textbf{Preprocessing:} The system generates a data preview $\Preview$, as indicated by the blue highlights in the figure.
%     \item \textbf{Schema Grounding:} This component maps the natural language intents to specific schema elements based on $\Preview$:
%     \begin{itemize}[leftmargin=*]
%         \item \textit{team} $\rightarrow$ \textsf{Player.Team} | \textsf{League.Team}
%         \item \textit{player} $\rightarrow$ \textsf{Player.Name} | \textsf{Player.PID}
%         \item \textit{best player} $\rightarrow$ \textsf{Player.Achievements}
%         \item \textit{year 2021} $\rightarrow$ \textsf{Player.Year} | \textsf{League.Season}
%         \item \textit{UCL} $\rightarrow$ \textsf{League.League}
%         \item \textit{win championship} $\rightarrow$ \textsf{Player.Achievements}
%     \end{itemize}
%     \item \textbf{Diversification:} Setting $K=3$, the system identifies three distinct strategies to resolve semantic ambiguity, such as checking if the year's \textit{top scorer} or a specific \textit{award winner} secured the UCL title.
%     \item \textbf{Decomposition:} The planner breaks the query into three alternative logical plans, depicted in Figure~\ref{fig:running_example_decomposition}. Due to inherent ambiguities in the query, the plans vary in how they define `best' and how they apply the temporal constraint to the specified conditions. Following decomposition, the plan is topologically sorted and validated for acyclicity; if it contains cycles, it is rejected.
%     \item \textbf{Optimization:} Next, the planner refines the generated plans for execution efficiency, as illustrated in Figure~\ref{fig:running_example_decomposition}. The optimizer prioritizes early pruning by pushing down relational filters and projections when possible. It defers semantic operators--particularly the semantic join, which, as the most expensive operation, is delayed longer than maps or filters.
%     \item \textbf{Execution:} Finally, the plan is executed by routing each step to its respective engine. Relational operations are translated into SQL and executed on the database, while semantic steps are dispatched to specialized execution engines. The resulting tables are then written back to the database.
%     \item \textbf{Consolidation:} Each plan reflects a different interpretation: Plan 1 selects Messi (2021 Ballon d'Or) and returns 0 as PSG did not win the championship; Plan 2 selects Jorginho (UEFA Player of the Year) and returns True following Chelsea's victory; Plan 3 selects Lewandowski (2021 Bundesliga top scorer) and returns True based on his career UCL titles. Ultimately, the final result depends on the chosen consolidation strategy.
% \end{itemize}
 
% \end{runningexample}

==> 4_preprocessing.tex <==
\section{Preprocessing}\label{sec:preprocessing}
The initial stage of $\System$ involves a comprehensive preprocessing of the database instance. This procedure is partitioned into two components: {a query-agnostic phase that normalizes and augments the database schema, and a query-aware phase that constructs a query-specific view of the data.}

% \begin{runningexample}
% The system generates a data preview $\Preview$, as indicated by the blue highlights in Figure~\ref{fig:planning}.
% \end{runningexample}

%(i) query-agnostic operations, which include general cleaning, structural normalization, and schema enrichment; and (ii) query-aware data preparation, which tailors the context specifically to the input question $\Question$. The following sections detail each preprocessing phase:
% \vspace{-0.5em}
\subsection{Query-agnostic Preprocessing}
The query-agnostic step is executed once per database instance to ensure structural integrity and reduce noise before any planning begins. This phase focuses on three key areas:

\begin{itemize}[leftmargin=*]
    \item \textbf{Table Cleaning and Normalization:} Enterprise schemas often contain structural inconsistencies such as duplicate attributes, malformed columns, or noisy fields. \System first performs normalization and cleaning to resolve such issues and ensure that downstream SQL execution remains reliable.
    
    %We resolve structural anomalies and duplicate attributes that may cause SQL parsing failures or ambiguous join paths. 
    \item \textbf{Heuristic Schema Pruning:} Many real-world schemas contain attributes that provide little semantic value for query processing (e.g., hash strings, identifiers with constant values, or columns dominated by NULL values). To reduce planning complexity and token overhead, \System eliminates columns where: (i) NULL values exceed a 95\% threshold, (ii) a single constant value dominates the attribute, or (iii) values contain non-informative content such as password hashes, Base64 strings, or code blocks. %Removing these ``junk'' attributes is critical, as high-entropy or binary-encoded strings can confuse LLM-based reasoning and exhaust the context window with non-semantic data and affect the planning fidelity and reliability.
    \item \textbf{Schema Augmentation:} To improve schema grounding during planning, the system augments the cleaned schema with lightweight data profiles (summarized in Table~\ref{tab:schema_augmentation}). These  include inferred attribute types, statistical summaries, and relational constraints such as primary and foreign keys. 
    
    % We enrich the remaining schema with data profiles, including inferred data types, primary and foreign key constraints, and type-specific statistical summaries. This augmentation provides the planner with the relational grounding necessary to generate well-typed and logically valid query plans. 
    % The specific data profiles extracted for each attribute category are summarized in Table~\ref{tab:schema_augmentation}.
\end{itemize}

\begin{table}[t]
\scriptsize
\centering
\caption{\small Data Profiling for Schema Augmentation}
\vspace{-1em}
\label{tab:schema_augmentation}
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{l|l|p{3.5cm}}
\toprule
\textbf{Attribute}  & \textbf{Relational}  & \textbf{Extracted Profile} \\
\textbf{Category}  & \textbf{Type Binding} & \textbf{Summaries} \\ \midrule
\textbf{Numeric}   & $\{\textit{int, float}\}$ & Min, Max, Average, Variance \\ \hline
\textbf{Categorical} & $\{\textit{string, enum}\}$ & Cardinality, Top-$k$ frequent values \\ \hline
\textbf{Textual}   & $\{\textit{varchar, text}\}$ & Min/Max length, unique count, sample snippets, semantic summaries \\ \hline
\textbf{Temporal}  & $\{\textit{date, timestamp}\}$ & Range [$t_{\textit{start}}, t_{\textit{end}}$], Granularity (e.g., year, day) \\ \hline
\textbf{Relational} & $\{\textit{PK, FK}\}$ & Referential constraints, join key mappings, table dependencies \\ 
\bottomrule
\end{tabular}
\vspace{-1.5em}
\end{table}
\subsection{Query-aware Preprocessing}

{While the previous phase improves schema quality, the planner still requires examples of the underlying data to accurately map natural language predicates to schema attributes. 
{This is particularly important for semi-structured tables where explicit attribute information may be unavailable.}
OmniTQA therefore constructs a query-aware data preview tailored to the input question $\Question$.}
% The query-aware phase executes a targeted distillation of the database context by leveraging the semantic intent of the input question $\Question$. 
This refinement is centered on two key primitives:
\begin{itemize}[leftmargin=*]
    \item \textbf{Semantic Schema Pruning:} This
    %While the initial agnostic cleaning removes structural noise, this
    step employs an LLM-based reasoning pass to identify and retain only those attributes likely relevant to the query intent. The goal is to significantly reduce the token overhead and minimize the potential for ``distraction'' during the subsequent phases.
    \item \textbf{Query-Aware Data Preview:} 
    %To provide the planner with concrete examples of the underlying data distribution, we construct a hybrid data preview $\Preview$. This involves a dual strategy:
    {This step constructs a hybrid preview $\Preview$ of the database content consisting of two components:}
     (i) \textit{Semantic Search}, which retrieves the top-$k_1$ rows most relevant to the question's predicates, and (ii) \textit{Random Sampling}, which includes $k_2$ random tuples to illustrate the general format and diversity of the relation. {This combination ensures that the planner receives both query-relevant examples and representative samples of the database structure, improving its ability to resolve predicates and attribute mappings.}
\end{itemize}

% Algorithm ~\ref{alg:preprocess} summarizes the preprocessing procedure. 
The output of this stage consists of a refined and context-augmented database instance $\Database^\Question$ and a query-aware data preview $\Preview$, which together serve as input for the planning and execution phases.

% The orchestration of the preprocessing phase is formalized in Algorithm~\ref{alg:preprocess}. The execution of this phase returns (i) a refined and context-augmented database instance $\Database^\Question$, and (ii) a query-aware data preview $\Preview$. These outputs serve as the grounded foundation for the downstream planning and execution phases.

% \begin{algorithm}[!tb]
% \small
% \caption{Pre-processing Phase of \System} \label{alg:preprocess}
% \begin{algorithmic}[1]
%     \Require Database $(\Schema, \Database)$, Question $\Question$, Parameters $k_1, k_2$
%     \Ensure Augmented Schema $\Database^\Question$, Query-Aware Preview $\Preview$
%     \Function{\textsc{Pre-Process}}{$\Schema, \Database, \Question, k_1, k_2$}
        
%         \State $\Schema_{norm}, \Database_{norm} \gets \textsc{NormalizeStructure}(\Schema, \Database)$ 
%         \State $\Schema_{cln} \gets \textsc{SchemaCleaning}(\Schema_{norm}, \Database_{norm})$
%         \State $\mathcal{M} \gets \textsc{ExtractProfiles}(\Schema_{cln}, \Database_{norm})$
        
%         \State $\Schema_{pruned} \gets \textsc{SemanticSchemaPruning}(\Schema_{cln}, \Question)$
%         \State $\Database^\Question \gets \Schema_{pruned} \cup \mathcal{M}$
        
%         \State $\Database_{sim} \gets \textsc{SemanticSearch}(\Database_{norm}, \Question, k_1)$
%         \State $\Database_{rand} \gets \textsc{RandomSample}(\Database_{norm}, k_2)$
%         \State $\Preview \gets \Database_{sim} \cup \Database_{rand}$
        
%         \State \Return $\Database^\Question, \Preview$
%     \EndFunction
% \end{algorithmic}
% \end{algorithm}


==> 5_planning.tex <==
% \vspace{-1em}
\section{Planning}\label{sec:planning}

{The planning phase consists of three main components: \textit{schema grounding}, \textit{atomic step decomposition}, and \textit{plan optimization.} Figure~\ref{fig:planning} illustrates the system components using a toy example.
% , while Algorithm~\ref{alg:planning_pipeline} details the formal workflow.}
In the following, we dive into the details of each component.}

\begin{figure*}[t]
  \centering
  \includegraphics[width=\textwidth]{figures/running_example.pdf}
  \vspace{-2.0em}
%     \caption{\small \System planning phase on \textsf{UEFA Soccer} database given query \textit{``Did the player who achieved the UEFA Men's Player of the Year 2021 win the UCL championship?''}. \System generates a data preview $\Preview$ (in blue) that is used to map NL intents to schema attributes. The planner generates and optimizes three distinct logical plans to resolve ambiguities, i.e., which column actually contains the information about UEFA Men's Player of the Year. Each plan represents a different schema interpretation: Plan A (Column ``Remark'' contains the information) and Plan B (Column ``Description'' contains), resulting in different execution outputs.}
    \caption{\small Illustration of the \System planning phase for the \textsf{UEFA Soccer} database and the query \textit{``Did the player who achieved the UEFA Men's Player of the Year 2021 win the UCL championship?''}. \System first constructs a query-aware data preview $\Preview$ (shown in blue) to ground natural-language intents to schema attributes. The planner then generates and optimizes multiple candidate logical plans to resolve the schema ambiguity over which column encodes the UEFA Men's Player of the Year information. For example, Plan A assumes the information is stored in column ``Remark'', whereas Plan B assumes it is stored in column ``Description'', yielding different execution outputs.}
  \vspace{-1em}
  \label{fig:planning}
\end{figure*}

% \begin{algorithm}[!tb]
% \small
% \caption{The \System Planning Pipeline} \label{alg:planning_pipeline}
% \begin{algorithmic}[1]
%     \Require Query $\Question$, Data Preview $\Preview$, Thresholds $\varepsilon, \tau, K$
%     \Ensure Plan Set $\mathbb{P} = \{\mathcal{G}^*_1, \dots, \mathcal{G}^*_k\}$
    
%     \Function{\textsc{GeneratePlans}}{$\Question, \Preview, K$}
%         \State $\mathbb{P} \gets \emptyset$;\quad $\Schema_{ground} \gets \textsc{GroundSchema}(\Question, \Preview)$
        
%         \State \texttt{// Cross-reference query intent with data distributions to find $K$ strategies}
%         \State $\mathbb{H} \gets \textsc{IdentifyStrategies}(\Question, \Preview, K)$ 
        
%         \For{each $\textit{strategy} \in \mathbb{H}$}
%             \State $\mathcal{G} \gets \textsc{Decompose}(\Question, \Schema_{ground}, \textit{strategy})$
%             \State $\mathcal{G}_{sorted}, \textit{hasCycle} \gets \textsc{TopologicalSort}(\mathcal{G})$
            
%             \If{$\neg \textit{hasCycle}$}
%                 \State $\mathcal{G}^* \gets \textsc{OptimizePlan}(\mathcal{G}_{sorted}, \varepsilon, \tau)$;\quad $\mathbb{P} \gets \mathbb{P} \cup \{\mathcal{G}^*\}$
%             \EndIf
%         \EndFor
%         \State \Return $\mathbb{P}$
%     \EndFunction
% \end{algorithmic}
% \end{algorithm}


% \vspace{-1em}
% \vspace{-0.5em}
\subsection{Schema Grounding}

{The first step is to map the entities and predicates expressed in $\Question$ to elements of the refined database schema. It operates at two levels:}

% The planning module initiates the generation of the execution plan by binding the abstract entities and logical predicates expressed in $\Question$ to the refined database schema. This \textit{schema grounding} procedure is essential for mitigating LLM hallucinations within the generated plan, and it operates at two distinct levels of granularity:

\begin{itemize}[leftmargin=*]
    \item \textbf{Relation-Level:} 
    % The system first identifies the minimal subset of base relations $\Relation_i \in \Schema$ necessary to evaluate $\Question$. By analyzing the query intent against the context-augmented schema, the planner actively prunes irrelevant tables. This ensures to only retain the required relational context, effectively bounding the search space for plan generation.
    {The system first identifies the subset of relations $\Relation_i \in \Schema$ required to answer $\Question$. Using the query-aware schema representation produced during preprocessing, the planner prunes irrelevant tables and retains only those that are likely to participate in the query plan.}

    
    \item \textbf{Attribute-Level:} Within the resolved relations, the planner maps NL descriptors to specific attributes $A \in \Attr$. This step heavily leverages the query-aware data preview $\Preview$ to bridge lexical gaps (e.g., mapping the phrase ``customer feedback'' to a specific column named \texttt{usr\_cmnt}).
\end{itemize}

{By grounding query expressions in concrete schema elements, the planner reduces hallucinations and ensures that the generated execution steps remain consistent with the database schema.}

% \begin{runningexample}
% This component maps the natural language intents to specific schema elements based on $\Preview$:
%     \begin{itemize}[leftmargin=*]
%         \item \textit{team} $\rightarrow$ \textsf{Player.Team} | \textsf{League.Team}
%         \item \textit{player} $\rightarrow$ \textsf{Player.Name} | \textsf{Player.PID}
%         \item \textit{best player} $\rightarrow$ \textsf{Player.Achievements}
%         \item \textit{year 2021} $\rightarrow$ \textsf{Player.Year} | \textsf{League.Season}
%         \item \textit{UCL} $\rightarrow$ \textsf{League.League}
%         \item \textit{win championship} $\rightarrow$ \textsf{Player.Achievements}
%     \end{itemize}
% \end{runningexample}
% \vspace{-0.5em}
\subsection{Atomic Step Decomposition}

Once the relevant schema elements are identified, the planner decomposes  $\Question$ into a sequence of \textit{atomic} reasoning steps. Each step $s$ represents a minimal executable unit that transforms one or more input relations into a new intermediate relation. To simplify execution and optimization, each atomic step satisfies two constraints:

\begin{itemize}[leftmargin=*]
    \item It contains at most one logical condition (e.g., $ \sigma_{col \theta val} $ where $\theta \in \{=, <, >, \dots\}$).
    \item The condition involves a single column or variable.
\end{itemize}
{This ensures that complex queries can be expressed as compositions of simple operations that are easier to interpret and optimize. } {The planner leverages statistical summaries and sample snippets within the preview $\Preview$ to resolve filter constants, identify valid join keys, and determine the mapping logic for semantic operators.}

% Throughout this decomposition, the planner leverages the query-aware data preview $\Preview$ to synthesize precise operational parameters. Specifically, the planner utilizes the statistical summaries and sample snippets within $\Preview$ to resolve exact filter constants, identify valid join keys, and determine the appropriate mapping logic for semantic operators.

The resulting steps are organized as DAG, denoted by $G = (V, E)$ where $V$ represent the set of atomic steps and $E$ represents directed dependencies between relations. A directed edge $(u, v) \in E$ implies a strict precedence constraint where step $u$ must be successfully completed before step $v$ can be initiated. This provides two advantages. First, it allows independent steps to be executed in parallel. Second, it provides an interpretable lineage of intermediate results that can be inspected or verified by users. {The planner then applies \textit{topological sort} $G$ to transform the DAG into a valid execution sequence. In the process, any plans with cycles are dropped and group of nodes that can be executed in parallel are also identified.}

% \begin{runningexample}
%     The planner breaks the query into three alternative logical plans, depicted in Figure~\ref{fig:planning}. Due to inherent ambiguities in the query, the plans vary in how they define `best' and how they apply the temporal constraint to the specified conditions.
% \end{runningexample}

% Once the execution plan is generated, a \textit{topological sort} is performed on $G$. This process is critical since it transforms the partial ordering of the DAG into a valid execution sequence, ensuring that no task is started until all its prerequisites are satisfied. Additionally by grouping nodes with an identical ``in-degree'' or depth during the sorting process, we can identify batches of tasks that are mutually independent and can be safely run in parallel. Finally, a valid execution plan must be acyclic. If the sorting algorithm fails to visit all $|V|$ nodes, it indicates the presence of a directed cycle. In such instances, the plan is logically unsound, and the system must ignore or reject the plan to prevent execution failure.

% \subsection{Anatomy of An Atomic Step}
% \vspace{-0.5em}
\subsection{Hybrid Operator Model}

{Each atomic step corresponds to an operator drawn from a predefined set of relational and semantic operators $O$ (depicted in Table~\ref{tab:operators}) . This hybrid operator model extends classical relational query processing by incorporating semantic reasoning capabilities.}
{Relational operators correspond to traditional database operations.
% such as scan, filter, projection, join, aggregation, sorting, and set operations. 
These operators are executed directly by the database engine and provide efficient data filtering and transformation. Semantic operators perform reasoning over textual attributes and are executed by an LLM-based reasoning module. These operators include semantic filtering (e.g., based on natural language condition), semantic mapping (e.g., derives structured values from textual fields), semantic joins (e.g., using fuzzy entity matching) and semantic aggregation (e.g., to summarize textual content).}
% nikita -- some of it is repetitive from previous sections, so rewriting slightly. also trying to improve connection to previous section 
% Following the decomposition of the NL query $\Question$ into a DAG, we define the internal composition of the constituent atomic steps. Each node in the execution plan represents a discrete operation $O$, mapping one or more input relations (either from the base schema $\Schema$ or intermediate results from preceding steps) to a resultant relation. 
% We categorize these operations into two distinct classes: (i) \textit{relational operators}, which are deterministic, high-performance relational primitives executed directly by the database engine; and (ii) \textit{semantic operators}, which leverage LLMs to handle probabilistic tasks such as fuzzy matching, sentiment extraction, and unstructured data synthesis. Table~\ref{tab:operators} provides the details of this hybrid operator universe. By extending classical relational primitives with their semantic counterparts, our proposed algebra provides a closed and complete system for reasoning over hybrid relational schemas under standard set semantics. 
Each step in the execution plan is represented as an object consisting of the following fields:
\begin{itemize}[leftmargin=*]
    \item \textsf{ID:} A unique identifier that serves as the symbolic name for the resultant relation $\Instance_{\textit{ID}}$ produced by the step.
    \item \textsf{Operator:} Specifies the operator name and class to be applied.
    \item \textsf{Instruction:} The grounded instantiation of the operator's \textit{instruction template}, tailored to the specific attributes $A \in \Attr$ and predicates $\textit{cond}$ required by the step.
    \item \textsf{Parents:} A list of antecedent step IDs representing the data dependencies within the DAG; these provide the input relations $\Instance_{a}, \Instance_{b}$ for the current operation.
\end{itemize}

{Unlike prior systems where semantic operators act over predefined schema attributes, in \System these operators also serve to recover latent relational structure from textual data, enabling subsequent symbolic processing.}

\begin{table*}[ht]
\scriptsize
\centering
\caption{\small The \System Operator Universe}
\vspace{-1em}
\label{tab:operators}
\renewcommand{\arraystretch}{1.4}
\begin{tabular}{l|l|l|p{4cm}|p{6cm}}
\toprule
\textbf{Class} & \textbf{Operator} & \textbf{Function} & \textbf{Instruction Template} & \textbf{Description} \\ \midrule
\multirow{8}{*}{\rotatebox[origin=c]{90}{\textbf{Relational}}} 
 & \textsf{SCAN}      & $\sigma(\Instance)$ & \textit{``Return rows from $\Instance$.''} & Retrieve base relation instance $\Instance_i \in \Database^\Question$. \\ \cline{2-5} 
 & \textsf{FILTER}    & $\sigma_{\textit{cond}}(\Instance)$ & \textit{``Return rows from $\Instance$ where $A$ [Op] $V$.''} & Select tuples $\Tuple \in \Instance$ where $A \in \AttrS$ meets a condition. \\ \cline{2-5} 
 & \textsf{PROJECT}   & $\pi_{A_1, \dots, A_k}(\Instance)$ & \textit{``Return $\{A_1, \dots, A_k\}$ of $\Instance$.''} & Projection over a subset of attributes $\{A_j\} \subseteq \AttrRel$. \\ \cline{2-5} 
 & \textsf{AGGREGATE} & $\gamma_{\textit{f}(A), \textit{G}}(\Instance)$ & \textit{``Return $\textit{f}(A)$ grouped by $\textit{G}$ from $\Instance$.''} & Deterministic reductions for $A \in \AttrS$ grouped by $\textit{G}$. \\ \cline{2-5} 
 & \textsf{JOIN}      & $\Instance_a \bowtie_{\theta} \Instance_b$ & \textit{``Return combined rows from $\Instance_a, \Instance_b$ via $\theta$.''} & Join operation based on exact key matching $\theta$. \\ \cline{2-5} 
 & \textsf{SORT}      & $\tau_{A}(\Instance)$ & \textit{``Return $\Instance$ sorted by $A$.''} & Reorder tuples $\Tuple \in \Instance$ by scalar values of attribute $A \in \AttrS$. \\ \cline{2-5} 
 & \textsf{LIMIT}     & $\lambda_{n}(\Instance)$ & \textit{``Return the top $n$ rows from $\Instance$.''} & Truncate the instance to the first $n$ tuples. \\ \cline{2-5} 
 & \textsf{SET\_OP}   & $\Instance_a \{ \cup, \cap, \setminus \} \Instance_b$ & \textit{``Return the [Op] of $\Instance_a$ and $\Instance_b$.''} & Standard set operations between compatible relations. \\ \hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{Semantic}}} 
 & \textsf{MAP} & $\tilde{\pi}_{\textit{cond}}(\Instance)$ & \textit{``Return $\Instance$ with new col derived from $\AttrU$ by \textit{cond}.''} & Row-wise transform (e.g., sentiment or entity extraction from $A \in \AttrU$). \\ \cline{2-5} 
 & \textsf{FILTER} & $\tilde{\sigma}_{\textit{cond}}(\Instance)$ & \textit{``Return rows from $\Instance$ satisfying \textit{cond}.''} & Probabilistic tuple selection based on fuzzy NL intent. \\ \cline{2-5} 
 & \textsf{JOIN}   & $\Instance_a \tilde{\bowtie}_{\textit{cond}} \Instance_b$ & \textit{``Join $\Instance_a, \Instance_b$ via matching logic: \textit{cond}.''} & Fuzzy entity resolution across relations via semantic similarity. \\ \cline{2-5} 
 & \textsf{AGGREGATE}    & $\tilde{\gamma}_{\textit{f}(A), \textit{G}}(\Instance)$ & \textit{``Return summary of $\AttrU$ grouped by $\textit{G}$ from $\Instance$ via \textit{cond}.''} & Synthesis or summarization of textual content in $\AttrU$. \\ \bottomrule
\end{tabular}
\vspace{-1em}
\end{table*}
% \vspace{-1.25em}
% \vspace{-0.5em}
\subsection{Plan Optimization}

{The execution plan generated by the planner may not be cost-efficient, particularly when semantic operators are involved. \System extends classical relational query optimization techniques ~\cite{selinger1979access, hellerstein1993predicate} to account for the asymmetry between inexpensive relational operations and expensive semantic reasoning. Specifically, we adopt predicate migration as a \textit{cost-aware semantic placement} strategy. While semantic operators are deferred to later stages to minimize unnecessary LLM calls, the optimizer evaluates the \textit{cardinality impact} of downstream relational operators. If a join or set operation is expected to significantly increase the number of tuples, semantic filters are applied earlier on smaller base relations to avoid costly expansion. The optimizer applies the following transformations:}
% So far, the resulting plan is a DAG, where each node represents an atomic step within our closed operator universe and each edge encapsulates the relational dependency between successive steps. Nevertheless, the resulting plan may lack the cost-optimality required for high-performance execution. Query optimization is a known NP-hard problem, and even identifying guaranteed near-optimal plans remains computationally difficult~\cite{chatterji2002complexity}.
% The complexity arises because execution costs fluctuate significantly across semantically equivalent plans. To address this, our optimizer prioritizes operator reordering to minimize the global execution cost, leveraging established algebraic identities—specifically commutativity, associativity, and distributivity—to transform the DAG without altering the result set. 

% We apply these optimization heuristics across several operator classes:

\begin{itemize}[leftmargin=*]
    \item \textbf{Selection Pushing:} 
    {When possible, relational filters are pushed toward the base relations to eliminate irrelevant tuples early in the plan.}
    %Relational selections are pushed down toward the data sources to minimize cardinality at the earliest possible stage. By reducing the number of tuples $\Tuple$ early, we minimize the data volume passed to downstream operators.
    
    \item \textbf{Projection Pruning:} 
    {Unnecessary attributes are removed once they are no longer required by downstream operations. This reduces the width of intermediate relations and memory footprint.}
    % nikita -- sacrificing some details to keep it succinct. add back if needed.
    %Projections are pushed down to remove unnecessary attributes $A$ as soon as they are no longer required for subsequent joins or filters. This reduces the tuple width and memory footprint, which is particularly vital for semantic operations where LLM context windows are limited and token-based costs are high.
    
    \item \textbf{Join Reordering:} 
    {Join operations are reordered to prioritize high-selectivity joins and minimize intermediate relation sizes.}
    
    % nikita -- sacrificing some details to keep it succinct. add back if needed.
    % Leveraging the commutativity and associativity of the join operator, we reassociate join sequences to prioritize those with the highest selectivity. This reordering ensures that the intermediate relation sizes are kept minimal. For joins involving semantic components, we attempt to evaluate symbolic predicates first to reduce the cross-product size before applying expensive semantic matching logic.
    
    \item \textbf{Adaptive Semantic Deferral:} Semantic steps are deferred until relational pruning is complete, unless a relational operator threatens to expand the result set, in which case the semantic step is prioritized to act as a pre-filter.
\end{itemize}

To formalize these heuristics, we define our join reordering strategy within the optimization framework shown in Algorithm~\ref{alg:optimizer}. For join reordering (\textsc{ReorderJoins}), we employ a threshold-based hybrid strategy that balances optimality and scalability. When the number of base relations is small ($|\mathcal{R}| \le \tau$), we use dynamic programming to search the space of left-deep join trees and obtain the cost-optimal plan. For larger queries, we fall back to a greedy heuristic that iteratively selects the relation minimizing intermediate join cost.
% For join reordering ((identified via \textsc{ReorderJoins})), we employ a threshold-based hybrid strategy to balance optimality with compile-time scalability. For queries containing a manageable number of base relations ($|\mathcal{R}| \le \tau$), we utilize a bottom-up Dynamic Programming algorithm to exhaustively search the plan space of left-deep trees, guaranteeing the cost-optimal relational structure. However, because dynamic programming scales exponentially, queries exceeding the $\tau$ threshold fall back to a deterministic Greedy heuristic. This greedy approach iteratively constructs the plan by selecting the next relation that yields the lowest intermediate join cost, ensuring scalable and predictable optimization even for highly complex queries.
% For the conditional deferral of semantic steps, we formalize our cost model $\mathcal{C}$ to account for both relational overhead and the distinct latency and token costs introduced by semantic operators. For a given query plan DAG $\mathcal{G}$, the total estimated execution cost is the sum of the costs of its constituent operators:
To guide semantic operator placement, we define a cost model that captures both relational execution cost and LLM inference cost. For a query plan DAG $\mathcal{G}$, the total estimated execution cost is:
$$Cost(\mathcal{G})=\sum_{o \in \mathcal{G}}\Big(w_{sys} \cdot C_{sys}(o)+w_{llm} \cdot C_{llm}(o)\Big)$$
where $w_{sys}$ and $w_{llm}$ are weighting factors. For relational operators, $C_{llm}(o)=0$, and the system cost $C_{sys}(o)$ is defined by traditional I/O and CPU estimates:
$$C_{sys}(o)=\gamma_{in}(o) \cdot c_{cpu}+pages(o) \cdot c_{io}$$
where $\gamma_{in}(o)$ denotes the estimated input cardinality for operator $o$. For a set operation like UNION ($A \cup B$), the output cardinality $\gamma_{out}$ is simply the additive sum of its inputs ($|A| + |B|$). For a join operator $A \bowtie B$, the input cardinality is the sum of the sizes of the two relations ($|A| + |B|$), while the output cardinality $\gamma_{out}$ (which becomes the input $\gamma_{in}$ for subsequent operators) is estimated using the selectivity of the join key:
$$\gamma_{out} = \frac{|A| \cdot |B|}{\max(| \pi_{key}(A) |, | \pi_{key}(B) |)}$$ 
where $| \pi_{key}(R) |$ represents the number of distinct values of the join attribute in relation $R$. This value is typically maintained in the system catalog, estimated via HyperLogLog sketches during data ingestion or periodic statistics updates~\cite{chen2017two, muller2021memory}. The parameters $c_{cpu}$ is the calibrated unit costs for CPU cycles per tuple,  $c_{io}$ is I/O disk page fetches and $pages(o)$ is total data volume in memory pages required for the operation.

% Crucially, for semantic operators, the cost is dominated by the LLM invocation. We model this as a function of the input cardinality and the average token length of the evaluated attributes $A$:
For semantic operators, the dominant cost arises from LLM inference. We model this as:
$$C_{llm}(o)=\gamma_{in}(o) \cdot \Big(c_{call}+\alpha \cdot \mathbb{E}[|tokens(A)|]\Big)$$
where $c_{call}$ denotes the base API latency, $\alpha$ is the marginal processing cost per token, and $\mathbb{E}[|tokens(A)|]$ is the expected token length of the evaluated attributes. This formulation motivates \textit{Adaptive Semantic Deferral}: minimizing the input cardinality $\gamma_{in}(o)$ through relational pruning directly reduces the LLM inference cost $C_{llm}(o)$. 

Rather than computing exact costs for every placement, the optimizer relies on a calibrated threshold $\varepsilon$ that captures the break-even point between relational data expansion and expensive LLM inference. It further considers the cardinality impact of downstream operators. Let $\Delta\gamma=\gamma_{out}/\gamma_{in}$ denote the ratio between the estimated output cardinality of a downstream operator and the input cardinality of the semantic branch. If $\Delta \gamma > \varepsilon$ (where $\varepsilon \ge 1$), the downstream join or set operation acts as a data multiplier. In such cases, executing the semantic filter earlier on the smaller base relation prevents a multiplicative increase in LLM token consumption.


% Let $\Delta \gamma$ be the ratio of the operator's total estimated output tuples to the input tuples flowing from the semantic operator's branch (i.e., $\Delta \gamma=\gamma_{out}/\gamma_{branch\_in}$). 
% The output cardinality $\gamma_{out}$ is estimated using traditional database metadata, such as primary/foreign-key relationships and histogram-based selectivity. 
% If $\Delta \gamma > \varepsilon$ (where $\varepsilon \ge 1$), the downstream join or set operation acts as a data multiplier. In such cases, executing the semantic filter earlier on the smaller base relation prevents a multiplicative increase in LLM token consumption.

The cost model parameters are obtained through a lightweight calibration phase. Relational parameters ($c_{cpu},c_{io}$) are estimated using synthetic workloads, while semantic parameters ($c_{call},\alpha$) are measured from LLM API latency and token statistics. Expected token lengths are maintained in the system metadata catalog.
%Relational constants ($c_{cpu}, c_{io}$) are profiled using synthetic scan and join workloads on the host hardware. Semantic constants are calibrated by sampling the LLM provider's response latency; $c_{call}$ represents the base network overhead (RTT), while $\alpha$ is the marginal latency per token. Average token lengths $\mathbb{E}[|tokens(A)|]$ are maintained as part of the system's metadata catalog, updated during data ingestion via a lightweight sampling tokenizer.

\begin{algorithm}[!tb]
\small
\caption{Heuristic-Based Plan Optimization of \System} \label{alg:optimizer}
\begin{algorithmic}[1]
    \Require Plan $\mathcal{G}$, Thresholds $\varepsilon, \tau$
    \Ensure Optimized Plan $\mathcal{G}^*$
    
    \Function{\textsc{OptimizePlan}}{$\mathcal{G}, \varepsilon, \tau$}
        \State $\mathcal{G}_{pushed} \gets \textsc{PushSelections}(\mathcal{G})$
        \State $\mathcal{G}_{pruned} \gets \textsc{PruneProjections}(\mathcal{G}_{pushed})$
        
        \State $\mathcal{G}_{ordered} \gets \textsc{ReorderJoins}(\mathcal{G}_{pruned}, \tau)$
        
        \For{each semantic node $v_{sem} \in \mathcal{G}$}
            \State $v_{down} \gets \textsc{GetNext}(v_{sem})$
            
            \If{$v_{down} \text{ is a \textsf{JOIN} } A \bowtie_{k} B$}
                \State $\gamma_{out} \gets (|A| \cdot |B|) / \max(| \pi_{key}(A) |, | \pi_{key}(B) |)$
            \ElsIf{$v_{down} \text{ is a \textsf{UNION} } A \cup B$}
                \State $\gamma_{out} \gets |A| + |B|$
            \EndIf
            
            \If{$v_{down} \text{ is a \textsf{JOIN} or \textsf{UNION}}$}
                \State $\Delta \gamma \gets \gamma_{out} / \gamma_{in}(v_{sem})$
                \If{$\Delta \gamma > \varepsilon$}
                    \State $\mathcal{G} \gets \textsc{Elevate}(v_{sem}, v_{down})$
                \Else
                    \State $\mathcal{G} \gets \textsc{Defer}(v_{sem})$
                \EndIf
            \EndIf
        \EndFor
        
        \State $\mathcal{G}^* \gets \mathcal{G}_{ordered}$
        \State \Return $\mathcal{G}^*$
    \EndFunction
    \Statex

    \Function{\textsc{ReorderJoins}}{$\mathcal{G}, \tau$}
        \State $\mathcal{R} \gets \mathcal{G}.\Schema$
        
        \If{$|\mathcal{R}| \le \tau$}
            \State $\mathcal{G}.\text{join\_tree} \gets \textsc{DP}(\mathcal{R})$ 
        \Else
            \State $\mathcal{G}.\text{join\_tree} \gets \textsc{Greedy}(\mathcal{R})$ 
        \EndIf
        
        \State \Return $\mathcal{G}$
    \EndFunction
    \Statex
    
    \Function{\textsc{Greedy}}{$\mathcal{R}$}
        \State $(\Relation_i, \Relation_j) \gets \arg\min_{\Relation_x, \Relation_y \in \mathcal{R}} \textsc{Cost}(\Relation_x \bowtie \Relation_y)$
        \State $Plan \gets \Relation_i \bowtie \Relation_j; \quad \mathcal{R} \gets \mathcal{R} \setminus \{\Relation_i, \Relation_j\}$
        
        \While{$\mathcal{R} \neq \emptyset$}
            \State $\Relation_{next} \gets \arg\min_{\Relation_k \in \mathcal{R}} \textsc{Cost}(Plan \bowtie \Relation_k)$
            \State $Plan \gets Plan \bowtie \Relation_{next}; \quad \mathcal{R} \gets \mathcal{R} \setminus \{\Relation_{next}\}$
        \EndWhile
        
        \State \Return $Plan$
    \EndFunction
    \Statex
    
    \Function{\textsc{DP}}{$\mathcal{R}$}
        \State $Opt \gets \emptyset$
        \For{each $\Relation_i \in \mathcal{R}$} 
            \State $Opt[\{\Relation_i\}] \gets \Relation_i$ 
        \EndFor
        
        \For{$size \gets 2$ \textbf{to} $|\mathcal{R}|$}
            \For{each subset $S \subseteq \mathcal{R}$ \textbf{where} $|S| = size$}
                \State $Opt[S] \gets \arg\min_{\Relation \in S} \textsc{Cost}(Opt[S \setminus \{\Relation\}] \bowtie \Relation)$
            \EndFor
        \EndFor
        
        \State \Return $Opt[\mathcal{R}]$
    \EndFunction
    \Statex
    
    \Function{\textsc{Cost}}{$A \bowtie B$}
        \State $\gamma_{in} \gets |A| + |B|$;\quad $pages \gets \textsc{EstimatePages}(A, B)$
        
        \State \Return $\gamma_{in} \cdot c_{cpu} + pages \cdot c_{io}$
    \EndFunction
\end{algorithmic}
\end{algorithm}

{In summary, Algorithm~\ref{alg:optimizer} rewrites an initial logical plan into a cost-optimized physical plan. It first applies rule-based transformations such as filter and projection pushdown, then performs hybrid join reordering, and finally determines semantic operator placement using the cost-aware deferral heuristic.}

{While our cost model provides a practical approximation of hybrid execution cost, it is not intended to be fully precise. Instead, it serves as a lightweight decision mechanism to guide operator placement and plan optimization. Empirically, we observe that even coarse-grained estimates are sufficient to achieve significant cost reductions, suggesting that precise modeling of LLM behavior may not be necessary for effective optimization.}

% In summary, Algorithm~\ref{alg:optimizer} rewrites an initial logical plan into a cost-optimized physical plan. It first applies rule-based transformations, including filter and projection pushdown, to reduce intermediate results early. It then employs a hybrid join reordering strategy to further constrain the search space. Finally, a cost-aware semantic deferral mechanism determines the placement of LLM operators, balancing execution efficiency with semantic evaluation requirements. With the plan now structurally and semantically optimized, it is ready to be passed to the execution engine.
% \vspace{-0.5em}
\subsection{Plan Diversification}

Although the optimizer identifies the cost-optimal plan under a given interpretation, natural language ambiguity in schemas and the probabilistic behavior of LLM-based semantic operators introduce a risk of \textit{semantic invalidity}. A plan may be structurally correct yet misaligned with the table semantics due to ambiguous schema mappings or model interpretation. To mitigate this, \System employs a \textit{Plan Diversification} strategy. Instead of committing to a single execution path, the planner generates a set of candidate plans  $\mathcal{P} = \{\mathcal{G}^*_1, \dots, \mathcal{G}^*_k\}$ that explore alternative schema mappings and operator configurations. This allows the system to hedge against incorrect assumptions during planning and resolve ambiguity through cross-plan comparison or user-guided refinement. We generate diversified plans along four dimensions:
% We categorize our diversification heuristics into four primary dimensions:

\begin{itemize}[leftmargin=*]
    \item \textbf{Schema Mapping Diversity:} {We map an ambiguous query term (e.g., `return player') to multiple candidate attributes (e.g., \texttt{player\_id} vs. \texttt{player\_name}).}
    
    %When a user's query term (e.g., \textit{``Find the 2021 league's top player.''}) is ambiguous relative to the schema, the system generates alternative plans targeting different candidate columns (e.g., \texttt{player\_id} vs. \texttt{player\_name}). This ensures that the system is not tethered to a single, potentially incorrect, attribute mapping.
    
    \item \textbf{Risk-Profile Variations:} {We generate  \textit{strict} plans that prioritize deterministic relational operators, and \textit{fuzzy} plans that use semantic operators to capture subjective predicates.}
    
    %We categorize candidate plans into \textit{Strict} and \textit{Fuzzy} execution paths to balance the trade-off between deterministic precision and semantic recall. Strict plans prioritize standard relational operators (e.g., \texttt{CONTAINS}, \texttt{LIKE}) to achieve low-cost, high-precision matches on symbolic data. Conversely, Fuzzy plans utilize semantic \texttt{FILTER} operators to resolve subjective or open-ended predicates, incurring a higher computational cost to capture semantic nuances that traditional operators might overlook.
    
    \item \textbf{Operator Substitution:} {We explore equivalent logical transformations (e.g., semantic \texttt{FILTER} vs. semantic \texttt{MAP} followed by relational filtering).}
    
    % The system explores equivalent logical transformations with differing execution profiles. For instance, a semantic requirement can be realized via a semantic \texttt{FILTER} or a semantic \texttt{MAP} followed by a standard relational \texttt{FILTER}.
    
    \item \textbf{Semantic Intent Modeling:} We interpret vague expressions (e.g., ``top player'') using alternative semantic criteria (e.g., scored goals vs. player of the match).
    
    % In the presence of vague qualifiers (e.g., ``top player''), \System employs lateral thinking heuristics to generate plans representing distinct interpretations, such as prioritizing number of scored goals versus player of the match or other player stats.
\end{itemize}

% \begin{runningexample}
%     Setting $K=3$, the system identifies three distinct strategies to resolve semantic ambiguity, such as checking if the year's \textit{top scorer} or a specific \textit{award winner} secured the UCL title.
% \end{runningexample}

% -- nikita -- commenting out now in interest of space.
% \nb{Starting from the grounded schema context, the system enumerates $K$ diversification strategies, constructs a plan DAG for each strategy, verifies its validity, and applies the cost-based optimizer to produce executable physical plans.}

% Managing a diversified plan set requires a final consolidation phase to identify the most valid result. This process may be handled via direct user intervention or through the automated consolidation strategies we propose in Section~\ref{sec:consolidation}. These techniques ensure that the exploration of the semantic search space ultimately converges on a unified and reliable query response.

% \vspace{1em}
% To conclude this section, we formalize the integrated logic of the planning phase in Algorithm \ref{alg:planning_pipeline}, which orchestrates the transition from NL intent to a diversified set of optimized physical plans. This pipeline synthesizes the previously discussed stages: it first establishes a grounded schema context $\Schema_{ground}$, and then iteratively generates $K$ candidate plans. For each candidate, the system performs an atomic decomposition guided by specific diversification heuristics, validates the resulting DAG via topological sorting to ensure logical soundness, and finally applies the cost-based optimization framework and prepares it for execution. The specific components and workflow of the planning phase are further depicted in Figure~\ref{fig:planning}.

==> 6_execution.tex <==
% \vspace{-1.5em}
\section{Execution}\label{sec:execution}

{After generating the diversified plan set $\mathbb{P}$, \System executes each plan $\mathcal{G}^* \in \mathbb{P}$ according to the precedence constraints of the plan DAG, routing operators to the appropriate execution engine.}
% Upon generating the diversified plan set $\mathbb{P}$, \System executes queries using a dual-engine architecture that coordinates a relational database engine and an LLM-based reasoning engine. Each plan $\mathcal{G}^* \in \mathbb{P}$ is executed according to the precedence constraints defined by the plan DAG, routing operators to the appropriate engine based on their type. 
To maximize throughput, \System exploits two levels of parallelism: \textit{inter-plan} parallelism, which executes the $K$ candidate plans concurrently, and \textit{intra-plan} parallelism, which schedules independent DAG nodes simultaneously. The following sections describe the execution of relational and semantic operators.
% \vspace{-0.5em}
\subsection{SQL-based Execution}

{Relational operators are executed by the \textit{SQL-based execution engine}. Given a grounded operator instruction, the engine translates it into an executable SQL query using schema metadata and data previews $\Preview$ from predecessor relations, and executes it on the host database.} {To improve robustness against translation errors, \System incorporates an automated refinement loop. If execution fails, the SQL query, error message, and logical instruction are passed to a refinement module that rewrites the query. This process repeats until execution succeeds or a retry limit is reached. Successful outputs are materialized as intermediate relations.}

% % When an atomic step is categorized as a relational operator, it is dispatched to the \textit{SQL-based execution engine}. This engine operates through a two-stage generative and corrective pipeline:

% % \begin{itemize}[leftmargin=*]
% %     \item \textbf{Text-to-SQL Translation:} The engine consumes the grounded operator instruction alongside the schema metadata and data previews $\Preview$ of the immediate predecessor relations. A translation module synthesizes these inputs into a native SQL query, which is then dispatched to the host database for execution.
% %     \item \textbf{Iterative Query Refinement:} To ensure robustness against syntactic or schema-mapping errors, \System implements an automated feedback loop. If the database engine returns an execution error, the failing SQL statement, the associated error log, and the original logical instruction are passed to a \textit{Refinement Module}. This module performs a root-cause analysis to rewrite the query. This iterative process persists until the query executes successfully or a maximum retry threshold is reached.
% % \end{itemize}

% Upon successful execution, the resulting tuples are materialized as intermediate relations within the database.
% \vspace{-0.5em}
\subsection{LLM-based Execution}

{
Semantic operators are executed by the \textit{LLM-based reasoning engine}. A naive approach would pass the entire relation to the LLM, which does not scale due to context limits, while row-wise execution incurs excessive API calls.} {To balance reasoning quality and execution efficiency, \System employs an operator-aware batching strategy that partitions input relations into manageable chunks. Batches are processed in parallel. This enables scalable semantic reasoning over large datasets while controlling token usage and latency. Unlike prior work \cite{patel2025semantic}, \System robustly integrates this approach directly into the physical execution of its hybrid operator model. }

% Steps categorized as semantic operators are dispatched to the \textit{LLM-based Reasoning Engine}. In a naive execution model, the grounded operator instruction and the entirety of the parent relations are passed to an LLM-based agent. This agent performs the specified semantic transformation and returns a structured result set, which is subsequently materialized as an intermediate relation within the host database.

% However, such holistic reasoning suffers from significant scalability and reliability bottlenecks common in LLM architectures: (i) As the cardinality of input relations increases, LLMs exhibit ``context rot'' phenomena, where reasoning reliability degrades significantly. Furthermore, large-scale joins can lead to quadratic growth in input size, frequently exceeding the model's maximum context window, (ii) While row-level execution (invoking the LLM for each tuple $t \in \Instance$) avoids context overflow, it incurs $O(N)$ API invocations. In a high-volume database environment, the cumulative network latency and token-based costs of $N$ individual calls render this approach computationally and economically prohibitive.

% To resolve the tension between reasoning quality and execution efficiency, \System incorporates an operator-specific batching strategy. By aggregating tuples into discrete batches, the execution engine calibrates the trade-off between maximizing context-window utilization and minimizing the total number of high-latency API invocations. While batching for semantic operators has been previously discussed in the literature (e.g., \cite{patel2025semantic}\nima{add more.}), \System robustly integrates this approach directly into the physical execution of its hybrid operator universe. \nima{What can we say about this to better claim it as a contribution?} The following sections detail the batching logic applied across different semantic operator classes to maintain high throughput and reasoning reliability.
% \vspace{-0.5em}
\subsection{Operator-driven Batching}

{The execution engine treats semantic operators as block-based primitives and dynamically determines an effective batch size $\beta$ based on a user-defined token budget and estimated schema width. If the token footprint of a batch exceeds the budget, $\beta$ is reduced to prevent context overflow. This chunking strategy enables substantial intra-operator parallelism by dispatching multiple LLM calls concurrently. Depending on the operator type, the engine applies one of three batching strategies:}


% The execution engine treats semantic operators as block-based primitives, dynamically calculating an \textit{effective batch size} ($\beta$) for each operation. This size is constrained by a user-defined token budget and the estimated token footprint of the schema's width. If the calculated token footprint per row threatens to exceed the budget, \System conservatively reduces $\beta$ to prevent context overflow.
% Crucially, this chunking strategy unlocks massive \textit{intra-operator parallelism}. By partitioning relations into independent blocks, \System dispatches multiple LLM API calls concurrently, effectively hiding network latency. Once $\beta$ is established, the engine routes the data using one of three core batching strategies:

\begin{itemize}[leftmargin=*]
    \item \textsf{Semantic MAP} \& \textsf{FILTER}: 
    {These operators evaluate tuples independently. Input relations are partitioned into chunks processed asynchronously. To reduce output tokens, the LLM returns only derived values (for \textsf{MAP}) or row indices satisfying the predicate (for \textsf{FILTER}), which are then applied to the original relation.}
    % Because these operations evaluate rows without cross-tuple dependencies, partitioned chunks are dispatched entirely asynchronously and in parallel. Furthermore, to drastically reduce output token generation costs, \System strictly limits the LLM's output payload. For \textsf{MAP}, the engine only returns an array of the newly derived values which upon completion is concatenated to the original relation. For \textsf{FILTER}, only an array of 0-based integer \textit{indices} corresponding to rows that satisfy the semantic condition is returned which are then used to natively filter the original chunks and materialize the survivors.
    
    \item \textsf{Semantic JOIN}: 
    {To avoid loading the full Cartesian product into a single context window, \System performs a block nested-loop join over LLM calls. Input relations are streamed in blocks of size $\beta$, and each block pair is evaluated independently in parallel.}
    
    % To handle semantic joins without loading the full Cartesian product into a single LLM context window, \System implements a memory-efficient block nested loop join over the LLM API. The outer and inner relations are streamed in blocks of size $\beta$. The evaluation of any given block pair $(C_A, C_B)$ is completely decoupled, allowing the cross-product to be evaluated concurrently. The engine returns an object containing the successfully joined row pairs, which are then synchronized and materialized.
    
    \item \textsf{Semantic AGGREGATE}: 
    {For operators requiring global context, \System employs a recursive map-reduce strategy. Relations larger than $\beta$ are partitioned into chunks, partial aggregations are computed in parallel, and intermediate results are recursively reduced until a final aggregation is produced.}
    
    % For operations requiring global context (e.g., summarization), a linear scan is insufficient. \System employs a recursive map-reduce strategy. If the relation exceeds $\beta$, it is chunked into partial batches. At any given depth level, the \textit{partial aggregations} for all chunks are dispatched in parallel. The completion of a depth level acts as a synchronization barrier. The intermediate results form a new relation, which is recursively processed until the total tuple count falls below $\beta$. A final LLM invocation then computes the definitive \textit{final aggregation}.
\end{itemize}

Algorithm~\ref{alg:llm_batching} outlines the complete batched execution logic employed by the LLM-based reasoning engine of \System.

\begin{algorithm}[!tb]
\small
\caption{Batching Semantic Operators} \label{alg:llm_batching}
\begin{algorithmic}[1]
    \Require Operator $Op$, Instruction $I$, Input Relation $\Instance$, Token Budget $B_{max}$, Base Batch Size $b$, Token Cost per Row $t_{row}$
    \Ensure Result Relation $\Instance_{out}$
    
    \Function{\textsc{ExecuteSemantic}}{$Op, I, \Instance, B_{max}, b, t_{row}$}
        \State $\beta \gets \min\Big(b, \lfloor B_{max} / t_{row} \rfloor \Big)$; \quad
        $\Instance_{out} \gets \emptyset$
        
        \If{$Op = \textsf{MAP}$}
            \For{$i \gets 0$ \textbf{to} $|\Instance|-1$ \textbf{step} $\beta$}
                \State $C \gets \Instance[i : i+\beta]$; \quad
                $Col_{new} \gets \textsc{Map}(I, C)$
                \State $\Instance_{out} \gets \Instance_{out} \cup \{ C[j] \oplus Col_{new}[j] \mid j \in \{0, \dots, |C|-1\} \}$
            \EndFor
            
        \ElsIf{$Op = \textsf{FILTER}$}
            \For{$i \gets 0$ \textbf{to} $|\Instance|-1$ \textbf{step} $\beta$}
                \State $C \gets \Instance[i : i+\beta]$ ;\quad
                 $Indices \gets \textsc{Filter}(I, C)$
                \State $\Instance_{out} \gets \Instance_{out} \cup \{ C[j] \mid j \in Indices \}$
            \EndFor
            
        \ElsIf{$Op = \textsf{JOIN}$}
            \For{$i \gets 0$ \textbf{to} $|\Instance|-1$ \textbf{step} $\beta$}
                \State $C_A \gets \Instance[i : i+\beta]$
                \For{$j \gets 0$ \textbf{to} $|\Instance_B|-1$ \textbf{step} $\beta$}
                    \State $C_B \gets \Instance_B[j : j+\beta]$;\quad
                     $res \gets \textsc{Join}(I, C_A, C_B)$
                    \State $\Instance_{out} \gets \Instance_{out} \cup res$
                \EndFor
            \EndFor
            
        \ElsIf{$Op = \textsf{AGGREGATE}$}
            \State $\Instance_{out} \gets \textsc{Reduce}(I, \Instance, \beta, 0)$
        \EndIf
        
        \State \Return $\Instance_{out}$
    \EndFunction
    \Statex
    
    \Function{\textsc{Reduce}}{$I, \Instance, \beta, depth$}
        \If{$|\Instance| \le \beta$ \textbf{or} $depth > MAX\_DEPTH$}
            \State \Return $\textsc{Aggregate}(I, \Instance)$
        \EndIf
        
        \State $\Instance_{partial} \gets \emptyset$
        \For{$i \gets 0$ \textbf{to} $|\Instance|-1$ \textbf{step} $\beta$}
            \State $C \gets \Instance[i : i+\beta]$;\quad
             $res \gets \textsc{Aggregate}(I, C)$
            \State $\Instance_{partial} \gets \Instance_{partial} \cup res$
        \EndFor
        
        \State \Return $\textsc{Reduce}(I, \Instance_{partial}, \beta, depth + 1)$
    \EndFunction
\end{algorithmic}
\end{algorithm}
% \vspace{-0.5em}
\subsection{Plan Consolidation}\label{sec:consolidation}

Since \System generates $K$ candidate execution plans exploring alternative reasoning paths, the final stage consolidates their outputs into a single result relation. Depending on user preferences for transparency, cost, and accuracy, \System supports three consolidation strategies:

\begin{itemize}[leftmargin=*]
    \item \textbf{LLM-as-a-Judge Consensus~\cite{gu2024survey}:} 
    {An independent LLM evaluates candidate outputs by comparing them against the original query and representative samples of each plan's results. Using few-shot examples to calibrate the evaluation, the judge selects the output that best aligns with the user’s intent.}
    
    % To automate the selection of the optimal output, \System utilizes a meta-reasoning stage where an independent LLM instance serves as a jurisdictional judge. This agent is provided with the original NL query and the candidate instructions generated for each of the $K$ plans, alongside representative samples of their materialized results. To calibrate the judge's evaluation, the prompt is augmented with few-shot examples illustrating the mapping between specific queries and their corresponding plausible versus non-plausible plans. By synthesizing these inputs, the judge evaluates the semantic fidelity of each candidate relative to the user's intent, selecting the most representative relation to serve as the final output.
    
    \item \textbf{Semantic Majority Voting~\cite{chen2024more}:} 
    {An ensemble-based strategy that treats each materialized relation as a vote and selects the result that appears most frequently across independent plans.}
    
    % \System implements an ensemble-based consensus mechanism that operates over the full materialized relations produced by the $K$ candidate plans. By treating the resulting relations as the unit of voting, the engine identifies the output state that achieves the highest frequency across independent reasoning paths.
    
    \item \textbf{User-Centric Delegation:} 
    {All $K$ result relations are returned to the user along with execution metadata (e.g., token usage and reasoning trace). This is useful in exploratory settings where the ``correct'' semantic transformation is subjective.}
    
    % In this mode, \System maintains the full diversity of the candidate space. Rather than forcing a singular output, the engine returns all $K$ materialized result sets to the user, annotated with their respective execution metadata (e.g., token usage and reasoning trace). This is particularly useful in exploratory data analysis where the ``correct'' semantic transformation is subjective.
\end{itemize}

% In Section~\ref{sec:experiments}, we empirically evaluate these consolidation strategies to quantify their relative impact on reasoning accuracy across various workloads.
% Finally, algorithm~\ref{alg:overall_exec} illustrates the end-to-end process of the execution phase.

% \nb{We empirically evaluate these consolidation strategies to quantify their relative impact on accuracy across various workloads.}
% Algorithm~\ref{alg:overall_exec} summarizes the overall execution pipeline.}

% \begin{runningexample}
% Each plan reflects a different interpretation: Plan 1 selects Messi (2021 Ballon d'Or) and returns 0 as PSG did not win the championship; Plan 2 selects Jorginho (UEFA Player of the Year) and returns True following Chelsea's victory; Plan 3 selects Lewandowski (2021 Bundesliga top scorer) and returns True based on his career UCL titles. 
% \end{runningexample}

% \begin{algorithm}[!tb]
% \small
% \caption{The \System Execution Pipeline} \label{alg:overall_exec}
% \begin{algorithmic}[1]
%     \Require Plan set $\mathbb{P} = \{\mathcal{G}^*_1, \dots, \mathcal{G}^*_K\}$ of topologically sorted DAGs, Query $\Question$, Strategy $S$, Max retries $N$
%     \Ensure Result $\Instance_{out}$
    
%     \State $\mathcal{R}_{set} \gets \emptyset$
    
%     \For{each plan $\mathcal{G}^* \in \mathbb{P}$}
%         \For{each operator $op \in \mathcal{G}^*$}
%             \If{$op \in \text{Relational}$}
%                 \State $\phi \gets \textsc{TranslateToSQL}(op.I, op.R)$;\quad
%                 $tries \gets 0$
%                 \Repeat
%                     \State $\Instance_{op}, error \gets \textsc{Db}.\textsc{ExecuteSQL}(\phi)$
%                     \If{$error$}
%                         \State $\phi \gets \textsc{RefineSQL}(\phi, error, op.I)$
%                     \EndIf
%                     \State $tries \gets tries + 1$
%                 \Until{$error = \emptyset$ \textbf{or} $tries \ge N$}
%             \Else
%                 \State $\Instance_{op} \gets \textsc{ExecuteSemantic}(op, op.I, op.R)$
%             \EndIf
%         \EndFor
%         \State $\mathcal{R}_{set} \gets \mathcal{R}_{set} \cup \{\Instance_{last}\}$
%     \EndFor
    
%     \State $\Instance_{out} \gets \textsc{Consolidate}(\mathcal{R}_{set}, \Question, S)$
%     \State \Return $\Instance_{out}$
% \end{algorithmic}
% \end{algorithm}

==> 7_experiments.tex <==
% \vspace{-0.5em}
\section{Experimental Evaluation}
\label{sec:experiments}
% \subsection{Evaluation Plan}

{We evaluate \System along two dimensions: \textit{effectiveness} (answer accuracy) and \textit{efficiency} (token usage). We further conduct ablation studies to quantify the impact of key components and design choices.}
% We aim to evaluate \System with respect to both effectiveness and efficiency. The effectiveness experiments assess the accuracy of the results obtained while cost experiments evaluate the token usage. We further conduct an ablation study to isolate the impact of specific components and design choices, ensuring a clear understanding of what drives the system's performance.
Our evaluation addresses the following research questions:

\begin{itemize}[leftmargin=*]
    \item \textbf{RQ1:} How does \System perform across diverse tasks and varying levels of query complexity?
    \item \textbf{RQ2:} How does \System compare to baselines in terms of token cost?
    \item \textbf{RQ3:} How do key hyperparameters affect performance?
    %How does the cost, in terms of token usage, associated with our approach compare to established baselines?
    \item \textbf{RQ4:} What is the impact of individual design components on effectiveness and efficiency?
    %How do specific architectural and design choices contribute to the overall effectiveness and efficiency of the system?
\end{itemize}
% \vspace{-0.5em}
\subsection{Datasets}
To evaluate \System in realistic settings, we use a diverse suite of table question answering datasets that span a wide range of challenges, including variations in table size (short vs. long), query complexity (lookup vs. compositional), schema quality (clean vs. noisy), database structure (single vs. multi-table), and data representation (structured vs. semi-structured). We include the following real-world datasets:
\begin{itemize}[leftmargin=*]
    \item \textsf{RepairTQA} \cite{zhang2025same}: {A diagnostic benchmark with seven subsets covering simple lookups (S1), compositional queries (S3), long tables (S4, S5), and multi-table reasoning (M1, M2)}.
    \item \textsf{WikiSQL} \cite{zhong2017seq2sql}: 
    A foundational large-scale dataset of NL questions paired with SQL queries over single tables.
    \item \textsf{WikiTableQuestions} \cite{pasupat2015compositional}: A dataset of complex questions over semi-structured Wikipedia tables requiring multi-step reasoning, such as comparison and aggregation.
    \item \textsf{FeTaQA} \cite{nan2022fetaqa}: A free-form table QA dataset that requires generating descriptive answers based on retrieved information.
    \item \textsf{HybridQA} \cite{chen2020hybridqa}: A multi-hop QA dataset that requires integrating  information from structured tables and linked unstructured text. 
    \item \textsf{TAT-QA} \cite{zhu2021tatqa}: A financial domain dataset requiring complex numerical reasoning from hybrid contexts of tables and text.
\end{itemize}

For datasets containing unstructured text (\textsf{FeTaQA}, \textsf{HybridQA}, \textsf{TAT-QA}), we convert them into a semi-structured format by appending the associated text as an additional column to each row.
% \textsf{FeTaQA}, \textsf{HybridQA} and \textsf{TAT-QA} datasets incorporate unstructured text at either the table level or the row level. 
% To transform these into a semi-structured format, we systematically append the associated text as a supplementary column within each corresponding table row.
{We evaluate on 100 samples per dataset, except for \textsf{RepairTQA}-\textsf{M2}, where we use 50 samples. To manage cost, we run all effectiveness experiments using \textsc{Gemini-3-Flash-Preview}, and evaluate additional models on a challenging subset of \textsf{RepairTQA}. All datasets include gold-standard annotations used for evaluation.}

% To evaluate our system, we select 100 samples from each dataset, with the exception of the \textsf{RepairTQA}-\textsf{M2} subset, for which we utilize 50 samples. 
% To manage experimental costs, we conducted the full suite of effectiveness experiments using \textsc{Gemini-3-Flash-Preview} across all datasets. For the remaining models and experiments, we evaluated on a subset of the most challenging datasets from the \textsf{RepairTQA} benchmark as representative cases. Each dataset is paired with gold-standard annotations, which serve as the basis for our performance evaluation.

% \vspace{-0.5em}
\subsection{Baselines}
We evaluate \System against three baseline categories: purely LLM-based, Text-to-SQL, and hybrid approaches. 

\begin{itemize}[leftmargin=*]
\item \textsc{Direct-LLM}: Directly prompts an LLM to generate answers without explicit intermediate reasoning or structured execution.

\item \textsc{NL2SQL}: A two-stage pipeline where an LLM generates a SQL query from the question and schema, which is then executed by a database engine.

\item \textsc{Plan-of-SQLs}~\cite{nguyen2025pos}: 
Decomposes complex queries into sequential natural language steps, each translated into executable SQL, with intermediate results guiding subsequent steps.
%Decomposes complex queries into a sequence of atomic, executable NL steps. Each step is converted into a simple SQL command and executed, using intermediate results to guide subsequent planning and reduce hallucinations. 

\item \textsc{H-Star}~\cite{abhyankar2025h}: 
{A hybrid approach that routes operations between SQL and LLMs based on task type (e.g., numerical vs. semantic). It assumes explicit schema attributes and does not support multi-table reasoning.}

%An adaptive hybrid approach that performs table extraction and filtering before routing tasks. It directs numerical and aggregation tasks to a SQL engine while routing descriptive or relational reasoning to the LLM, thereby balancing symbolic computation with NL inference. This method is incapable of reasoning across multi-table settings and operates under explicit schema assumption.

\item \textsc{Weaver}~\cite{khoja2025weaver}: 
{A hybrid method that interleaves SQL execution with LLM reasoning in a stepwise pipeline. It relies on explicit schemas and does not generalize to multi-table or semi-structured settings.}
% utilizes a stepwise workflow to interweave SQL execution and LLM reasoning. It assigns specific operations to either the symbolic or neural engine and feeds intermediate results back into the plan. \textsc{Weaver} requires an explicit schema and does not work across multiple tables.
% \nb{TODO: this makes weaver sound very much like our own system. we can shorten the last line and instead talk about what it does not do.}
\end{itemize}

% \vspace{-0.5em}
% \subsection{Result Evaluation Protocol}
% To assess model performance against ground-truth annotations, we utilize an LLM-based evaluation framework rather than relying on exact string matching following the approach utilized for evaluating \textsf{RepairTQA} \cite{zhang2025same}. This judge-based approach accounts for syntactic and representation variations, such as differing row orders, container types (e.g., lists vs. tuples), and minor orthographic differences. This methodology is particularly advantageous for free-form generative tasks, where multiple semantically equivalent responses may be factually correct despite surface-level differences.
% % \nb{TODO: better to cite existing works and suggest we follow a standard evaluation protocol for this task.}

% \vspace{-0.5em}
\subsection{Experiment Settings}
% \subsubsection{Experimental Setup}

\System is implemented in Python 3.11. All experiments were conducted on a high-performance server equipped with an AMD EPYC 7R32 (48-core CPU), 192GB of RAM, and eight NVIDIA A100 GPUs. We evaluated multiple LLMs, including \textsc{Gemini-3-Flash-Preview}, \textsc{GPT-5-Mini}, and \textsc{Qwen3:30B}; with the latter deployed locally via \textsc{Ollama}. Embeddings are generated using the \texttt{all-MiniLM-L6-v2} encoder and cosine similarity was used for retrieval during the query-aware preprocessing step.
% \subsubsection{Parameter Settings} 
In the default configuration, we set the number of plans to $K=6$ and the batch size to $\beta=100$. {We study sensitivity by varying $K \in [1,6]$ and $\beta \in [10,1000]$. Unless otherwise stated, \textsc{Gemini-3-Flash-Preview} is used for all experiments. For fair comparison, all methods use the same underlying LLMs. We detail prompts utilized across \System in the supplemental technical report~\cite{techrep}.}
%To evaluate the impact of these hyperparameters, we perform sensitivity analyses by varying the number of plans $K$ from 1 to 6 and scaling the batch size $\beta$ across a range from 10 to 1000. For all comprehensive evaluations, \textsc{Gemini-3-Flash-Preview} serves as the default model. To ensure a fair comparison, we adapted the source code of all baseline methodologies to utilize the same LLMs as \System.

% \subsubsection{Evaluation Metrics} 
{We evaluate outputs using an LLM-based judge, following \textsf{RepairTQA}~\cite{zhang2025same}, instead of exact string matching. This approach accounts for variations in ordering, formatting (e.g., lists vs. tuples), and minor textual differences, and is well-suited for free-form outputs with semantically equivalent answers.}

% To assess model performance against ground-truth annotations, we utilize an LLM-based evaluation framework rather than relying on exact string matching following the approach utilized for evaluating \textsf{RepairTQA} \cite{zhang2025same}. This judge-based approach accounts for syntactic and representation variations, such as differing row orders, container types (e.g., lists vs. tuples), and minor orthographic differences. This methodology is particularly advantageous for free-form generative tasks, where multiple semantically equivalent responses may be factually correct despite surface-level differences.

\begin{summary}
{\System consistently achieves best performance across challenging settings, including large tables, complex compositional queries, and multi-relation schemas. It matches or exceeds state-of-the-art baselines on simpler tasks, while maintaining competitive token efficiency among hybrid approaches. These gains are consistent across different underlying LLMs.}
%\System consistently emerges as the top-performing system across a variety of challenging settings, including high-cardinality tables, complex compositional queries, and multi-relation schemas, outperforming competing systems by a substantial margin. For simpler lookup tasks or short tables, \System performs on par with or exceeds state-of-the-art baselines. Cost-wise, it maintains competitive cost efficiency compared to existing hybrid approaches while achieving significantly higher accuracy. Notably, these improvements remain consistent across different underlying LLMs.
\end{summary}

% \vspace{-0.5em}
\input{plots_1}
\subsection{RQ1: Effectiveness Results}

{We compare \System against all baselines under four configurations: Acc@6, Acc@1, Majority Voting, and LLM-as-a-Judge. Figures~\ref{fig:acc_gemini},~\ref{fig:acc_gpt}, and~\ref{fig:acc_qwen}, show that \System consistently outperforms baselines, with the largest gains observed on challenging tasks.}

%\nb{We begin by evaluating the overall effectiveness of \System across a diverse set of table reasoning tasks with varying complexity. This setup allows us to assess the system’s robustness and scalability under heterogeneous, real-world workloads. For each experiment, we compare \System against multiple baselines and report performance under four configurations: Acc@6 (top-of-6 candidates), Acc@1 (single-path execution), Majority Voting, and LLM-as-a-Judge.}

% Figures~\ref{fig:acc_gemini},~\ref{fig:acc_gpt}, and~\ref{fig:acc_qwen}, demonstrate the overall robustness of \System and its significant performance gains over established baselines, particularly in more challenging tasks. 


{\stitle{Direct LLM methods}  These methods performs competitively on simpler tasks involving small tables and look up queries (e.g., \textsf{RepairTQA-S1}, \textsf{WikiSQL}, \textsf{WikiTableQuestions}, \textsf{FeTaQA}, and \textsf{HybridQA}\footnote{Strong performance on Wikipedia-derived benchmarks may partly stem from pre-training data contamination.}. However, its performance degrades significantly as task difficulty increases with long tables (\textsf{RepairTQA-S4}), complex queries (\textsf{RepairTQA-S3}, \textsf{RepairTQA-S5}), and multi-table settings (\textsf{RepairTQA-M1}, \textsf{RepairTQA-M2}). While effective for unstructured reasoning, it struggles with scale and multi-hop integration.}

% \vspace{-0.5em}
\stitle{Text-to-SQL methods} {\textsc{NL2SQL} and \textsc{Plan-of-SQLs} underperform on most benchmarks, except \textsf{WikiSQL}, where schemas are simple and well-structured. Their limitations stem from an inability to reason over unstructured text and relying on basic string-matching operators native in SQL.}

% \nb{\textsc{NL2SQL} and \textsc{Plan-of-SQLs} generally underperform across benchmarks, with the exception of \textsf{WikiSQL}, where simple and uniform schemas make the task more tractable.}
% Their limitations stem from an inability to effectively handle unstructured textual columns. They are typically limited to basic string-matching operators native in SQL, which are insufficient for capturing the semantic nuances required for complex reasoning over unstructured content.
% \vspace{-0.5em}
\stitle{Hybrid baselines} {\textsc{H-Star} and \textsc{Weaver} achieve moderate performance but lack native support for semi-structured inputs. They remain competitive on structured datasets but exhibit sensitivity to the underlying LLM. We also observed that the performance does not consistently generalize across benchmarks.}
% State-of-the-art hybrid baselines, such as \textsc{H-Star} and \textsc{Weaver}, achieve moderate performance on semi-structured datasets but lack native support for such inputs. \nb{They remain competitive on fully structured data but exhibit strong sensitivity to the underlying base model.} 
% Notably, \textsc{Weaver} exhibits significant performance degradation when integrated with \textsc{Qwen} models, whereas \textsc{H-Star} performs suboptimally under \textsc{GPT} architectures. 
%These methods also exhibit dataset-specific biases; while \textsc{Weaver} performs reasonably well on the \textsc{RepairTQA} benchmark, it fails to generalize to other semi-structured datasets.}
% \vspace{-0.5em}

\stitle{\System} {\System consistently achieves the best performance across all semi-structured datasets.  Under LLM-as-a-Judge, it ranks first in 6/9 settings and remains within a small margin in the remaining cases. Gains over the next-best method are substantial, reaching up to 48\% on \textsf{RepairTQA-M2} and 39\% on \textsf{RepairTQA-S5}. On structured datasets, \System performs on par with leading baselines (within $\sim$3\%). These trends remain consistent across different underlying LLMs.}

{
% We assessed the performance of \System using four consolidation strategies: Accuracy@6 (an upper bound measuring if any of the six plans succeed), Accuracy@1 (the precision of a single plan), Majority Voting, and LLM-as-a-Judge. 
While $\text{Accuracy@6}$ yields the highest accuracy, it relies on ground-truth labels or human supervision, limiting its practicality in real-world deployment. In contrast, LLM-as-a-Judge emerges as the most effective practical strategy by consistently achieving near-top performance. Majority voting performs similarly and typically trails the LLM-based judge by a small margin. Finally, $\text{Acc@1}$ performs worst across all settings, highlighting the importance of generating and evaluating multiple candidate plans.}

%Even when considering consolidated results using LLM-as-a-judge, \System ranks as the top-performing method in six out of nine configurations; while in the three remaining settings, it trails the top-performing baseline by only a marginal delta. Performance gains over the next best method are substantial in several cases, reaching as high as 48\% for \textsf{RepairTQA-M2} and 39\% for \textsf{RepairTQA-S5}. For structured datasets, \System performs on par with the leading approach, exhibiting a performance gap of only approximately 3\%.
% Importantly, these findings are largely independent of the underlying base model, as consistent performance trends are observed across different architectures.

\stitle{Remark} A manual audit of \System’s performance on \textsf{RepairTQA} reveals that most failures are approach-agnostic and stem from dataset limitations, including incorrect labels, ambiguous questions, and structural issues such as missing or incomplete data. Additionally, the semantic evaluation protocol occasionally produces false negatives. While such benchmark noise is well documented~\cite{wretblad-etal-2024-understanding}, we retain these cases to ensure a consistent and unbiased comparison. Excluding them would uniformly inflate performance across all methods.
%Furthermore, a non-trivial portion of errors is attributable to the semantic evaluation protocol, which occasionally produces false negatives. While the literature acknowledges such benchmark noise~\cite{wretblad-etal-2024-understanding} and it is common practice to identify these limitations, we retain these samples to ensure a rigorous and unbiased comparison across all methodologies. Excluding these instances would result in a substantial, uniform increase in accuracy across all evaluated approaches.

\subsection{RQ2: Efficiency Results}

We evaluate the computational cost of \System in terms of token consumption. Input and output tokens are reported separately (stacked bars), with darker segments indicating input tokens and lighter segments output tokens. We report total cost for generating and executing one and six plans, with the latter representing an upper bound. Costs for Majority Voting and LLM-as-a-Judge are omitted as they closely match the six-plan setting.  All results are aggregated over the full evaluation set.%Furthermore, we report the aggregate cost of processing the entire dataset across all evaluated benchmarks.

Figures~\ref{fig:cost_gemini},~\ref{fig:cost_gpt} and~\ref{fig:cost_qwen} show that \System achieves higher accuracy and robustness at a cost comparable to or lower than existing hybrid methods.
%achieves superior robustness and accuracy at a cost that is either comparable to or lower than that of existing hybrid approaches, while simultaneously outperforming them by a substantial margin. 
Moreover, the execution cost of a single plan is on par with the \textsc{Direct-LLM} baseline. Conversely, Text-to-SQL methodologies--particularly \textsc{NL2SQL}--remain the most cost-effective, as their overhead is limited to processing data previews and generating SQL queries. Finally, we observed that across all settings, input tokens dominate the total cost.

%Finally, we evaluate the relationship between batch size ($\beta$) and computational cost. The general trend illustrated in Figure~\ref{fig:varying_beta_cost} demonstrates that as the batch size increases, the associated costs decrease significantly. This reduction is primarily attributable to the increased efficiency of batched processing, which results in fewer API calls to the LLM and a reduction in the redundant processing of shared prompt overhead.

\subsection{RQ3: Hyperparameters Sensitivity}
We next examine how hyperparameters influence the effectiveness and efficiency of \System. For these and all following experiments, we employ \textsc{Gemini-3-Flash-Preview} as the base model.

\stitle{Number of Plans ($K$)}
We analyze the effect of varying the number of plans ($K$) on accuracy (Figure~\ref{fig:varying_k_acc}). We observed that accuracy improves as $K$ increases, with the largest gain observed from $K=1$ to $K=2$, after which performance plateaus. This suggests that a small number of plans already captures most of the benefit, and further increases yield diminishing returns relative to cost.

In terms of cost, as shown in Figure~\ref{fig:varying_k_cost}, total cost scales linearly with $K$, since each additional plan incurs a full generation and execution cycle.



%In this experiment, we evaluate the impact of the number of plans ($K$) on accuracy, as illustrated in Figure~\ref{fig:varying_k_acc}. While accuracy scales with the number of plans, the marginal improvement is most pronounced when transitioning from one to two plans, after which performance begins to plateau. This suggests that in scenarios with limited budget, generating a limited number of plans yields highly competitive results; beyond this point, the diminishing returns in accuracy may not justify the linear increase in cost.

\stitle{Batch Size ($\beta$)}
Next, we evaluate the impact of varying the batch size ($\beta$) on the accuracy of \System. As illustrated in Figure~\ref{fig:varying_beta_acc}, accuracy generally decreases as $\beta$ increases, with more pronounced degradation at larger values, likely due to longer contexts introducing noise or hallucinations. These results highlight the importance of empirically tuning $\beta$; such optimization could be performed via expert manual intervention or through a small-scale validation (e.g., binary search over a representative subset).

Regarding the impact on cost, Figure~\ref{fig:varying_beta_cost} shows that cost decreases with larger $\beta$, due to more efficient batching that reduces the number of LLM calls and eliminates the redundant processing of shared prompt overhead.

% \subsubsection{Impact on Efficiency}
% \paragraph{Number of Plans ($K$)}
% \nb{As shown in Figure~\ref{fig:varying_k_cost}, total cost scales linearly with $K$, since each additional plan incurs a full generation and execution cycle.}
% %Next, we analyze the relationship between the number of plans and the overall cost. As illustrated in Figure~\ref{fig:varying_k_cost}, the total token consumption scales linearly with the number of plans, as each additional plan necessitates a complete cycle of generation and execution.

% \vspace{-0.5em}
% \paragraph{Batch Size ($\beta$)}
% \nb{Figure~\ref{fig:varying_beta_cost} shows that cost decreases with larger $\beta$, due to more efficient batching that reduces the number of LLM calls and eliminates the redundant processing of shared prompt overhead.}

\input{plots_2}

\subsection{RQ4: Impact of Individual Components}

We conduct an ablation study to systematically quantify the contribution of key components in \System (Table~\ref{tab:ablation_combined}). We report accuracy results using Acc@6 (Table~\ref{tab:ablation_combined}.a) and LLM-as-a-judge(Table~\ref{tab:ablation_combined}.b). 

% \vspace{-1em}
{\stitle{Query-aware preview}
We replace the query-aware preview with a uniformly sampled subset of equivalent size from the underlying table. We observed that this leads up to  8\% accuracy drop (as reported in the `w/ Naive $\Preview$' column of Tables~\ref{tab:ablation_combined}.a and~\ref{tab:ablation_combined}.b). The effect is smaller for smaller tables, where relevant information is more likely to appear in random samples.}

%We begin by evaluating the impact of query-aware data previews. To isolate this effect, we replace the query-aware preview with a uniformly sampled subset of equivalent size from the underlying table. This modification results in a performance degradation of up to 8\% (as reported in the `w/ Naive $\Preview$' column of Tables~\ref{tab:ablation_combined}.a and~\ref{tab:ablation_combined}.b). Notably, the impact is less pronounced for smaller tables, where the probability of relevant predicates appearing in a random sample is statistically higher.

{\stitle{Schema pruning}
Disabling schema pruning results in up to 4\% degradation (reported in the ``w/o Pru. $\Schema$'' column). While modest on average, the impact is more pronounced on wide or noisy tables, where pruning reduces irrelevant attributes and improves grounding. Among these challenging instances, our heuristic successfully mitigated the noise, thereby preventing performance drops that would otherwise occur in more complex structural environments.
}
%Next, we evaluate the impact of our schema pruning heuristics on overall accuracy. The results, reported in the ``w/o Pru. $\Schema$'' column, demonstrate a performance degradation of up to 4\%. While this margin appears modest, it is significant given the data distribution: the benchmark contains a limited number of samples with exceptionally wide or noisy tables. Among these challenging instances, our heuristic successfully mitigated the noise, thereby preventing performance drops that would otherwise occur in more complex structural environments.

{\stitle{Operator model}
We replace our operator model with a QDMR-based decomposition~\cite{wolfson-etal-2020-break}. Since QDMR does not explicitly decouple semantic and relational operators, we introduce a routing agent that can direct each step to appropriate execution engine based on instructions and data previews. The resulting degradation in accuracy is significant across all settings, reaching as high as 49\%. This highlights that design of operators for \Problem is a non-trivial task and that it is important to separate semantic and relational operators for accurate decomposition in semi-structured settings.}

%Next, we evaluate the contribution of our operator model, specifically tailored for semi-structured tasks. To assess its impact, we compare the full implementation of \System against a baseline utilizing the established QDMR~\cite{wolfson-etal-2020-break} operator set. For this configuration, we not only modify the operator set but also introduce a routing agent responsible for directing each step to the appropriate execution engine based on step instructions and data previews; this is necessary because QDMR does not explicitly decouple semantic and deterministic (relational in this case) operators.
% The resulting degradation in accuracy is significant across all settings, reaching as high as 49\%. This finding demonstrates that the separation of operators into distinct groups--combined with adherence to relational algebra operators--exerts a substantial impact on decomposition accuracy. 

{\stitle{Plan Optimization} 
To assess the impact of plan optimization, we execute plans without optimization. The  corresponding accuracy and cost results are presented in the "w/o Opt $\mathcal{G}$" columns of Tables~\ref{tab:ablation_combined}.a, \ref{tab:ablation_combined}.b, and \ref{tab:ablation_combined}.c. Notably, accuracy remains invariant, verifying that our reordering strategy preserves the logical integrity of the plans. However, costs increase by up to 20\%. This confirms that our optimization strategy improves efficiency without affecting correctness.}

%The next component evaluated is our plan optimization methodology. To assess its impact, we compare our approach against a baseline that executes generated plans as-is, without optimization. The corresponding accuracy and cost results are presented in the "w/o Opt $\mathcal{G}$" columns of Tables~\ref{tab:ablation_combined}.a, \ref{tab:ablation_combined}.b, and \ref{tab:ablation_combined}.c. Notably, accuracy remains invariant, verifying that our reordering strategy preserves the logical integrity of the plans. However, the cost results reveal a significant improvement of up to approximately 20\%. These findings underscores the critical importance of plan optimization strategies in managing the high-volume, demanding workloads typical of corporate environments.

{\stitle{Plan Diversification}
We replace our plan diversification strategy with  naive generation of $K$ plans that delegates diversification entirely to the LLM's inherent lateral thinking capabilities. The results, presented in the "w/o Div. $\mathcal{G}$" column, reveal an accuracy decline of up to 18\%, indicating that stochastic LLM variation is insufficient and a structured diversification of plans is instead necessary.}

%Lastly, we evaluate the impact of our plan diversification strategies. To isolate this effect, we replace our tailored, query-and-workload-specific strategy selection with a baseline that generates $K$ plans in an agnostic manner, delegating diversification entirely to the LLM's inherent lateral thinking capabilities. The results, presented in the "w/o Div. $\mathcal{G}$" column, reveal an accuracy decline of up to 18\%. This significant drop highlights that relying solely on stochastic model variation is insufficient, and underscores the necessity of carefully steering diversification strategies for achieving high performance.
%\vspace{-0.5em}
\subsection{Error Analysis}

{While many errors in \textsf{RepairTQA} benchmark arise from data inconsistencies or evaluation protocol, \System also exhibits some approach-specific failures. We conduct a qualitative assessment of these failure cases to identify the potential sources of errors. We attribute errors into three sources: (i) schema grounding, (ii) planning, and (iii) execution (Figure~\ref{fig:error_analysis}).}

%As previously mentioned, errors in the \textsf{RepairTQA} benchmark are typically not approach-specific; instead, they often stem from data inconsistencies or the result-matching procedure. Nonetheless, cases exist where \System fails to capture the correct answer. This section provides a qualitative analysis to identify and investigate the root causes of these failures. Approach-specific errors are categorized by their source: (i) schema grounding, (ii) planning, or (iii) execution. The results of this qualitative evaluation are presented in Figure~\ref{fig:error_analysis}. 

{\stitle{Planning errors} The majority of failures originate in planning. A common issue is incomplete projections, where not all requested attributes are returned (e.g., omitting middle names when `full name' is requested). Another frequent failure arises when the planner lacks exposure to dataset-specific values. In these cases, it may hallucinate alternatives (e.g., substituting \textsf{status}=`extinct' with `inactive' or `disappeared'). This also leads to incorrect operator choices. For example, planner can fail to interpret the specific literal `northern california' and semantically map the city to a region value instead that does not exist in the underlying data. This also manifest sometimes as incorrect interpretation of the query intent (e.g., treating `most verbose complaint' as word count instead of service duration. }

%Our key observation is that the majority of approach-specific errors arise from planning failures. A prevalent instance of such errors involves the final projection, where \System occasionally fails to include all requested columns in the result set despite being logically plausible. For example, given the query \textit{``Please list the full names of all the male clients born after the year 1990''}, the system returns only the first and last names, omitting the middle name despite its availability in the schema. 
% Another issue arises when the planner, lacking exposure to specific predicate conditions, fails to define correct filters and relies instead on internal knowledge. For instance, given the query \textit{``List names of coins that have disappeared,''} the planner may substitute the correct attribute value (\textsf{status}=`extinct') with hallucinated terms like `inactive' or `disappeared'. This lack of domain-specific value awareness can also lead to incorrect operator selection. For example, in the query \textit{``List all cities in the Northern California Region,''} the planner's failure to recognize the specific literal `northern california' causes it to semantically map the city to a region value that does not exist in the underlying data. Another instance involves misinterpretation of query terms. For example, in the query \textit{``On which day was the most verbose complaint received,''} the planner calculates word counts in the description field rather than identifying the record with the maximum service time, as intended by the domain logic.

{\stitle{Schema grounding errors} These occur when query terms are incorrectly mapped to schema attributes. For example, similarity between column names may lead to selecting \textsf{ProductCategoryID} instead of \textsf{ProductSubcategoryID}. In other cases, the system struggles with implicit semantics, such as mapping `has a text box' to a negated boolean field (\textsf{isTextLess}). Such schema grounding errors are well-known in Text-to-SQL systems, and can be sometimes resolved with sophisticated schema linking.}


% Schema grounding is the next most frequent error source, occurring when \System fails to map query terms to the intended columns. For example, in the query \textit{``Please provide the IDs of any three AdventureWorks product subcategories,''} the high similarity between column names causes the planner to incorrectly select \textsf{ProductCategoryID} instead of the requested \textsf{ProductSubcategoryID}. A further example is the query \textit{``Please list the names of the cards that have a text box.''} In this case, the planner fails to recognize that the \textsf{isTextLess} column represents the condition, struggling to map the presence of a feature to a negative boolean attribute.

{\stitle{Execution errors} Execution errors are less frequent and typically involve semantic operators. These include incorrect attribute extraction despite correct row retrieval (e.g., returning `province' instead of `country', as well as incomplete retrieval where valid rows are missed.}

% The least frequent error source is execution, typically involving semantic operators where the LLM hallucinates or misinterprets data. For example, in the query \textit{``Which country does Baghdad belong to?''}, the semantic engine identifies the correct record but fails to extract the country attribute. Instead, it erroneously returns the \textsf{province}, demonstrating a failure in attribute-specific retrieval despite correct step instruction and successful row localization. Furthermore, we observed that in some instances, the semantic executor exhibits incomplete retrieval, where valid rows are bypassed despite meeting the filter conditions. 

{\stitle{Robustness to data vs. prior knowledge} We further observe that the execution engine prioritizes database content over parametric knowledge. To evaluate this robustness, we performed a counterfactual analysis by altering the values associated with specific filters in several samples. For instance, in the query \textit{``List all cities in the Northern California Region,''} we replaced the relevant records with cities from New York. The the system faithfully returns modified data, indicating strong grounding to the input rather than memorized world knowledge.}

%Finally, we observed that the semantic execution engine prioritizes the underlying data over its internal knowledge. To evaluate this robustness, we performed a counterfactual analysis by altering the values associated with specific filters in several samples. For instance, in the query \textit{``List all cities in the Northern California Region,''} we replaced the relevant records with cities from New York. The executor remained loyal to the database state, returning the modified data despite its internal training and potential exposure to the correct real-world facts.





==> 8_related_works.tex <==
\section{Related Work}
\label{sec:related_work}

{\stitle{Text-to-SQL and Table QA} Text-to-SQL systems translate NL queries into executable SQL over structured schemas, achieving strong performance when all query-relevant information is explicitly represented \cite{luo2025survey,hong2025next,liu2024survey,deng2025reforce}. However, these methods remain limited to relational operators and largely assume that all required attributes are present in the schema. Table question answering methods \cite{zhang2025survey,yu-etal-2025-table,wu2025tablebench,wu2025mmqa} instead operate directly over tables, often treating them as serialized text and leveraging LLMs for reasoning. While flexible, these methods typically struggle with scalability, multi-table reasoning, and execution efficiency.}

\stitle{Semantic operator systems}
A growing body of work extends relational query processing with LLM-based semantic operators, enabling tasks such as semantic filtering, entity matching, and aggregation \cite{patel2025semantic,liu2025palimpzest,glenn2024blendsql,su2026large}. 
These approaches significantly enhance query expressiveness, but typically assume that schema attributes and relationships are explicitly defined. As a result, semantic operators are used to interpret or enrich existing data, rather than recover missing structure.

% The paradigm of database interaction is shifting from rigid query languages toward fluid, NL interfaces. In this regard, two primary bodies of work have gained significant attention: (1) \textit{Table Question Answering}, which strives to answer NL queries over structured relational databases, and (2) \textit{Document Intelligence}, which aims to answer questions regarding collections of multi-modal documents.

% Literature in Table QA generally follows two distinct trajectories: semantic parsing and direct tabular reasoning. Semantic parsing, often formulated as \textit{Text-to-SQL}, focuses on translating natural language into executable database queries. This approach heavily relies on robust schema linking and structural encoding to map utterances to relational schemas~\cite{luo2025survey}. Conversely, direct \textit{Tabular Reasoning} approaches bypass intermediate query generation. Instead, they serialize table contents or utilize pre-trained language models designed specifically to reason over tabular structures to extract or compute answers directly~\cite{zhang2025survey,yu-etal-2025-table}. A third line of research explores hybrid approaches, integrating both paradigms to mitigate their respective limitations~\cite{abhyankar2025h,khoja2025weaver}.

% Parallel to developments in structured data, research in document comprehension focuses on extracting answers from dense textual collections, such as PDFs, reports, and unstructured corpora \cite{maekawa2025holistic}. Earlier approaches framed this as a combination of \textit{Information Retrieval} and \textit{Machine Reading Comprehension}, establishing the ubiquitous retriever-reader architecture~\cite{chen2017reading, karpukhin2020dense}. As language models have scaled, the field has increasingly adopted \textit{Retrieval-Augmented Generation} paradigms to synthesize answers from retrieved document chunks~\cite{lewis2020retrieval, gao2023retrieval,maekawa-etal-2024-retrieval,taguchi-etal-2025-efficient}. Furthermore, advancements in long-context models now allow systems to process entire PDFs or lengthy unstructured texts directly in the prompt, mitigating the need for complex retrieval pipelines~\cite{xu2023retrieval}.

{\stitle{Hybrid semantic-symbolic pipelines.} Recent hybrid systems interleave symbolic database operations with LLM-based reasoning in stepwise pipelines~\cite{khoja2025weaver,abhyankar2025h}. These approaches route sub-tasks between relational engines and LLMs, enabling flexible query execution across heterogeneous data. However, they typically operate at a coarse granularity and rely on predefined schemas, limiting their ability to handle scenarios where relational structure is implicit or must be inferred from textual fields. They also have limited support for complex settings such as long tables, multi-tables and multi-hop queries. Furthermore, these approaches are optimized for a fixed data representation and do not generalize well to settings where schemas are hybrid or evolve over time~\cite{zhang2025same}.}

\stitle{Unstructured document processing} Research in document comprehension has transitioned from retriever-reader architectures \cite{chen2017reading, karpukhin2020dense} to Retrieval-Augmented Generation for synthesizing answers from unstructured data \cite{lewis2020retrieval, gao2023retrieval, maekawa2025holistic}. Recent long-context models further streamline this by processing extensive texts directly, potentially bypassing traditional retrieval pipelines \cite{xu2023retrieval}.

{\stitle{Semi-structured data processing.}
Prior work on semi-structured data has explored querying and extracting structure as well as integrating information extraction pipelines with databases \cite{sun2026knowledge,maekawa2025holistic}. However, these approaches assume that structure can be reliably extracted ahead of time and do not address settings where query-relevant structure is context-dependent or cannot be fully materialized in advance.
}

In contrast to prior work, \System targets settings where query-relevant structure is not explicitly materialized and must be reconstructed during query execution~\cite{chen2020hybridqa, zhang2025same}. This requires treating semantic reasoning not only as an augmentation to relational processing, but as a mechanism to recover latent schema elements and enable downstream symbolic reasoning. 

% While prior research has predominantly operated under one of these two isolated paradigms, modern enterprise data is inherently heterogeneous and a mixture of both. In practice, information is frequently distributed across multiple interconnected tables and databases, often embedding unstructured text within relational columns~\cite{chen2020hybridqa, zhang2025same}. Resolving NL queries in these environments requires robust semantic reasoning frameworks capable of navigating data noise and complex, multi-table schema dependencies.

% To the best of our knowledge, \System is the first system specifically designed to address NL questions within the context of semi-structured databases.
% \nima{Add more citations later.}

==> 9_conclusion.tex <==
\section{Conclusion}

{In this paper, we introduced \System, a hybrid query processing framework for semi-structured table question answering. \System integrates relational operators with LLM-based semantic reasoning by representing queries as DAGs of atomic operators executed across dual engines. It further incorporates data-aware planning and cost-based optimization to reduce expensive semantic computation, while generating multiple candidate plans to handle natural language ambiguity in the table schema.}
% In this paper, we introduced \System, a hybrid query processing framework designed to address the challenges of semi-structured table question answering. By recognizing that real-world enterprise databases often contain a mixture of structured attributes and free-form textual fields, \System interleaves deterministic relational operators with LLM-based semantic reasoning. \System decomposes NL queries into a structured execution plan consisting of a DAG of atomic steps. Each step corresponds to a predefined operator drawn from a finite universe of symbolic relational operators or LLM-based semantic operators. During execution, \System routes these operators to the appropriate execution engine: symbolic operators are compiled into SQL for database execution, while semantic operators are evaluated by an LLM-based executor. To navigate the inherent ambiguity of NL, \System generates multiple candidate plans to explore alternative semantic interpretations. Furthermore, the framework applies a cost-aware optimizer that prioritizes operator reordering and relational pruning to minimize expensive LLM-based reasoning.
Empirical evaluations across several benchmark datasets demonstrate that \System consistently outperforms state-of-the-art baselines in terms of accuracy while maintaining competitive cost efficiency. It shows largest gains on complex queries, large tables, and multi-relation settings.

%It proves particularly superior for complex queries, high-cardinality tables, and multi-table settings where all classes of baselines tend to underperform.

{Despite these advances, challenges remain in planning quality, cost, and latency. In particular, generating diverse high-quality plans remains a bottleneck. Since optimization is inherently limited by the quality of the initial plan, incorporating human-in-the-loop to audit and prune plans could significantly improve reliability and cost-efficiency. Furthermore, semantic operators continue to incur significant overhead. A tiered execution approach involving a high-recall, efficient hash-based \textsf{FILTER} or \textsf{JOIN} to prune the search space prior to the more expensive LLM-based execution can be helpful. This can be further augmented by model cascading strategies, which utilize a hierarchy of models to route simpler logic to smaller, cost-effective models while reserving larger LLMs for complex reasoning tasks.}

% \nima{Despite current optimizations, bottlenecks still exist regarding system accuracy, cost, and latency. Planning remains a primary constraint, as LLM agents frequently struggle to generate high-quality, distinct alternatives for the same query even when employing diversification strategies; this lack of variance directly impacts overall accuracy. Furthermore, optimization is inherently limited by the quality of the initial plan, as an inefficient original execution path forces subsequent refinements to remain anchored to a high-cost baseline. To address this, a human-in-the-loop feature to audit and prune plans could significantly improve reliability and cost-efficiency. 
% Additionally, semantic steps remain computationally expensive and consume significant time and token budgets, even with the application of batching strategies. As a future work, we propose a tiered execution approach involving a high-recall, efficient hash-based \textsf{FILTER} or \textsf{JOIN} to prune the search space prior to the more expensive LLM-based execution. This can be further augmented by model cascading strategies, which utilize a hierarchy of models to route simpler logic to smaller, cost-effective models while reserving larger LLMs for complex reasoning tasks.}

As semi-structured data continues to proliferate, the architectural principles established by \System provide a scalable blueprint for the next generation of intelligent data interfaces.

==> plots_1.tex <==
\begin{figure*}[!tb] 
\centering
    \includegraphics[width=0.9\textwidth]{figures/legend.pdf}\\
    \begin{minipage}[t]{\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/accuracy_gemini.pdf}
        \vspace{-2.0em}
        \caption{\small Accuracy comparison of \System vs. baselines evaluated with \textsc{Gemini-3-Flash}.}
        \label{fig:acc_gemini}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.20\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/accuracy_gpt.pdf}
        \vspace{-2.0em}
        \caption{\small Accuracy comparison: \textsc{GPT-5-Mini}.}
        \label{fig:acc_gpt}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.20\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/accuracy_qwen.pdf}
        \vspace{-2.0em}
        \caption{\small Accuracy comparison: \textsc{QWEN3:30B}.}
        \label{fig:acc_qwen}
    \end{minipage}
    \hfill
    % \begin{minipage}[t]{0.20\linewidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figures/accuracy_gpt_5_4.pdf}
    %     \vspace{-2.7em}
    %     \caption{\small Accuracy comparison: \textsc{GPT-5.4}.}
    %     \label{fig:acc_gpt_5_4}
    % \end{minipage}
    % \hfill
    % \begin{minipage}[t]{0.20\linewidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figures/accuracy_gemini_3_1_pro.pdf}
    %     \vspace{-2.7em}
    %     \caption{\small Accuracy comparison: \textsc{Gemini-3.1-Pro}.}
    %     \label{fig:acc_gemini_3_1}
    % \end{minipage}
    % \hfill
    \begin{minipage}[t]{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/cost_gemini.pdf}
        \vspace{-2.0em}
        \caption{\small Cost comparison: \textsc{Gemini-3-Flash}.\protect\footnotemark}
        \label{fig:cost_gemini}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/cost_gpt.pdf}
        \vspace{-2.0em}
        \caption{\small Cost comparison: \textsc{GPT-5-Mini}.}
        \label{fig:cost_gpt}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/cost_qwen.pdf}
        \vspace{-2.0em}
        \caption{\small Cost comparison: \textsc{QWEN3:30B}.}
        \label{fig:cost_qwen}
    \end{minipage}
    % \hfill
    % \begin{minipage}[t]{0.19\linewidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figures/cost_gpt_5_4.pdf}
    %     \vspace{-2.7em}
    %     \caption{\small Cost comparison: \textsc{GPT-5.4}.}
    %     \label{fig:cost_gpt_5_4}
    % \end{minipage}
    % \hfill
    % \begin{minipage}[t]{0.19\linewidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figures/cost_gemini_3_1_pro.pdf}
    %     \vspace{-2.7em}
    %     \caption{\small Cost comparison: \textsc{Gemini-3.1-Pro}.}
    %     \label{fig:cost_gemini_3_1}
    % \end{minipage}
% %     \hfill
% %     \begin{minipage}[t]{0.19\linewidth}
% %         \centering
% %         \includegraphics[width=\textwidth]{figures/varying_num_of_plans_accuracy.pdf}
% %         \vspace{-2.7em}
% %         \caption{\small Varying no. of plans $K$ vs. accuracy.}
% %         \label{fig:varying_k_acc}
% %     \end{minipage}
% %     \hfill
% %     \begin{minipage}[t]{0.19\linewidth}
% %         \centering
% %         \includegraphics[width=\textwidth]{figures/varying_batch_size_accuracy.pdf}
% %         \vspace{-2.7em}
% %         \caption{\small Varying batch size $\beta$ vs. accuracy.}
% %         \label{fig:varying_beta_acc}
% %     \end{minipage}
% %     \hfill
% %     \begin{minipage}[t]{0.19\linewidth}
% %         \centering
% %         \includegraphics[width=\textwidth]{figures/varying_num_of_plans_cost.pdf}
% %         \vspace{-2.7em}
% %         \caption{\small Varying no. of plans $K$ vs. cost.}
% %         \label{fig:varying_k_cost}
% %     \end{minipage}
% %     \hfill
% %     \begin{minipage}[t]{0.19\linewidth}
% %         \centering
% %         \includegraphics[width=\textwidth]{figures/varying_batch_size_cost.pdf}
% %         \vspace{-2.7em}
% %         \caption{\small Varying batch size $\beta$ vs. cost.}
% %         \label{fig:varying_beta_cost}
% %     \end{minipage}
% %     \hfill
% %     \begin{minipage}[t]{0.19\linewidth}
% %         \centering
% %         \includegraphics[width=\textwidth]{figures/error_chart.pdf}
% %         \vspace{-2.7em}
% %         \caption{\small Error categorization in \textsf{RepairTQA}.}
% %         \label{fig:error_analysis}
% %     \end{minipage}
\vspace{-1em}
\end{figure*}
% % \footnotetext{Darker and lighter shades denote \textit{input} and \textit {output} tokens, respectively.}
% % \begin{table*}[t]
% % \footnotesize
% % \centering
% % \caption{\small Ablation Study}
% % \label{tab:ablation_combined}
% % \vspace{-1.5em}
% % \newcommand{\vhead}[1]{\rotatebox[origin=c]{90}{\textbf{#1}}}
% % \setlength{\tabcolsep}{3pt} % Tightens internal padding to ensure fit

% % % Shading definitions
% % \definecolor{sigdrop}{rgb}{1.0, 0.5, 0.5}
% % \definecolor{moddrop}{rgb}{1.0, 0.8, 0.8}
% % \definecolor{slidrop}{rgb}{1.0, 0.9, 0.9}

% % % --- First Table: Acc@6 ---
% % \begin{minipage}{0.30\textwidth}
% % \centering
% % \caption*{ (a) Accuracy (Acc@6)}
% % \vspace{-1.5em}
% % \begin{tabular}{l|c|ccccc}
% % \toprule
% % \textbf{Dataset} & \vhead{\System} & \vhead{w/ Naive $\Preview$} & \vhead{w/ QDMR} & \vhead{w/o Opt. $\mathcal{G}$} & \vhead{w/o Div. $\mathcal{G}$} & \vhead{w/o Pru. $\Schema$} \\ \midrule
% % \textsf{RepairTQA-S4} & \textbf{0.78} & \cellcolor{moddrop}0.70 & \cellcolor{sigdrop}0.53 & 0.78 & \cellcolor{moddrop}0.66 & \cellcolor{slidrop}0.77 \\ \hline
% % \textsf{RepairTQA-S3} & \textbf{0.86} & 0.86 & \cellcolor{sigdrop}0.57 & 0.86 & \cellcolor{moddrop}0.79 & \cellcolor{slidrop}0.83 \\ \hline
% % \textsf{RepairTQA-M1} & \textbf{0.86} & \cellcolor{moddrop}0.78 & \cellcolor{sigdrop}0.37 & 0.86 & \cellcolor{moddrop}0.72 & \cellcolor{slidrop}0.82 \\ 
% % \bottomrule
% % \end{tabular}
% % \end{minipage}% <--- THIS PERCENT IS CRITICAL
% % \hfill
% % % --- Second Table: LLM Judge ---
% % \begin{minipage}{0.30\textwidth}
% % \centering
% % \caption*{ (b) Accuracy (LLM-as-a-Judge)}
% % \vspace{-1.5em}
% % \begin{tabular}{l|c|ccccc}
% % \toprule
% % \textbf{Dataset} & \vhead{\System} & \vhead{w/ Naive $\Preview$} & \vhead{w/ QDMR} & \vhead{w/o Opt. $\mathcal{G}$} & \vhead{w/o Div. $\mathcal{G}$} & \vhead{w/o Pru. $\Schema$} \\ \midrule
% % \textsf{RepairTQA-S4} & \textbf{0.65} & \cellcolor{moddrop}0.59 & \cellcolor{sigdrop}0.43 & 0.65 & \cellcolor{moddrop}0.53 & 0.65 \\ \hline
% % \textsf{RepairTQA-S3} & \textbf{0.74} & 0.74 & \cellcolor{sigdrop}0.46 & 0.74 & \cellcolor{moddrop}0.68 & \cellcolor{slidrop}0.73 \\ \hline
% % \textsf{RepairTQA-M1} & \textbf{0.70} & \cellcolor{moddrop}0.64 & \cellcolor{sigdrop}0.33 & 0.70 & \cellcolor{moddrop}0.59 & \cellcolor{slidrop}0.68 \\ 
% % \bottomrule
% % \end{tabular}
% % \end{minipage}% <--- THIS PERCENT IS CRITICAL
% % \hfill
% % % --- Third Table: Cost ---
% % \begin{minipage}{0.25\textwidth}
% % \centering
% % \caption*{ (c) Cost}
% % \vspace{-1.5em}
% % \begin{tabular}{l|c|c}
% % \toprule
% % \textbf{Dataset} & \textbf{\System} & \textbf{w/o Opt. $\mathcal{G}$} \\ \midrule
% % \textsf{RepairTQA-S4} & \textbf{16.7M} & \cellcolor{moddrop}20.4M \\ \hline
% % \textsf{RepairTQA-S3} & \textbf{1.3M} & \cellcolor{moddrop}1.6M \\ \hline
% % \textsf{RepairTQA-M1} & \textbf{0.6M} & \cellcolor{slidrop}0.7M \\ 
% % \bottomrule
% % \end{tabular}
% % \end{minipage}
% \vspace{-0.5em}
% \end{table*}

==> plots_2.tex <==
\begin{figure*}[!tb] 
\centering
    % \includegraphics[width=0.9\textwidth]{figures/legend.pdf}\\
    % \begin{minipage}[t]{\linewidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figures/accuracy_gemini.pdf}
    %     \vspace{-2.7em}
    %     \caption{\small Accuracy comparison of \System vs. baselines evaluated with \textsc{Gemini-3-Flash}.}
    %     \label{fig:acc_gemini}
    % \end{minipage}
    % \hfill
    % \begin{minipage}[t]{0.20\linewidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figures/accuracy_gpt.pdf}
    %     \vspace{-2.7em}
    %     \caption{\small Accuracy comparison: \textsc{GPT-5-Mini}.}
    %     \label{fig:acc_gpt}
    % \end{minipage}
    % \hfill
    % \begin{minipage}[t]{0.20\linewidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figures/accuracy_qwen.pdf}
    %     \vspace{-2.7em}
    %     \caption{\small Accuracy comparison: \textsc{QWEN3:30B}.}
    %     \label{fig:acc_qwen}
    % \end{minipage}
    % \hfill
    % % \begin{minipage}[t]{0.20\linewidth}
    % %     \centering
    % %     \includegraphics[width=\textwidth]{figures/accuracy_gpt_5_4.pdf}
    % %     \vspace{-2.7em}
    % %     \caption{\small Accuracy comparison: \textsc{GPT-5.4}.}
    % %     \label{fig:acc_gpt_5_4}
    % % \end{minipage}
    % % \hfill
    % % \begin{minipage}[t]{0.20\linewidth}
    % %     \centering
    % %     \includegraphics[width=\textwidth]{figures/accuracy_gemini_3_1_pro.pdf}
    % %     \vspace{-2.7em}
    % %     \caption{\small Accuracy comparison: \textsc{Gemini-3.1-Pro}.}
    % %     \label{fig:acc_gemini_3_1}
    % % \end{minipage}
    % % \hfill
    % \begin{minipage}[t]{0.19\linewidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figures/cost_gemini.pdf}
    %     \vspace{-2.7em}
    %     \caption{\small Cost comparison: \textsc{Gemini-3-Flash}.\protect\footnotemark}
    %     \label{fig:cost_gemini}
    % \end{minipage}
    % \hfill
    % \begin{minipage}[t]{0.19\linewidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figures/cost_gpt.pdf}
    %     \vspace{-2.7em}
    %     \caption{\small Cost comparison: \textsc{GPT-5-Mini}.}
    %     \label{fig:cost_gpt}
    % \end{minipage}
    % \hfill
    % \begin{minipage}[t]{0.19\linewidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figures/cost_qwen.pdf}
    %     \vspace{-2.7em}
    %     \caption{\small Cost comparison: \textsc{QWEN3:30B}.}
    %     \label{fig:cost_qwen}
    % \end{minipage}
    % % \hfill
    % % \begin{minipage}[t]{0.19\linewidth}
    % %     \centering
    % %     \includegraphics[width=\textwidth]{figures/cost_gpt_5_4.pdf}
    % %     \vspace{-2.7em}
    % %     \caption{\small Cost comparison: \textsc{GPT-5.4}.}
    % %     \label{fig:cost_gpt_5_4}
    % % \end{minipage}
    % % \hfill
    % % \begin{minipage}[t]{0.19\linewidth}
    % %     \centering
    % %     \includegraphics[width=\textwidth]{figures/cost_gemini_3_1_pro.pdf}
    % %     \vspace{-2.7em}
    % %     \caption{\small Cost comparison: \textsc{Gemini-3.1-Pro}.}
    % %     \label{fig:cost_gemini_3_1}
    % % \end{minipage}
    % \hfill
    \begin{minipage}[t]{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/varying_num_of_plans_accuracy.pdf}
        \vspace{-2.0em}
        \caption{\small Varying no. of plans $K$ vs. accuracy.}
        \label{fig:varying_k_acc}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/varying_batch_size_accuracy.pdf}
        \vspace{-2.0em}
        \caption{\small Varying batch size $\beta$ vs. accuracy.}
        \label{fig:varying_beta_acc}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/varying_num_of_plans_cost.pdf}
        \vspace{-2.0em}
        \caption{\small Varying no. of plans $K$ vs. cost.}
        \label{fig:varying_k_cost}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/varying_batch_size_cost.pdf}
        \vspace{-2.0em}
        \caption{\small Varying batch size $\beta$ vs. cost.}
        \label{fig:varying_beta_cost}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/error_chart.pdf}
        \vspace{-2.0em}
        \caption{\small Error categorization in \textsf{RepairTQA}.}
        \label{fig:error_analysis}
    \end{minipage}
% \vspace{-1em}
\end{figure*}
\footnotetext{Darker and lighter shades denote \textit{input} and \textit {output} tokens, respectively.}
\begin{table*}[t]
\footnotesize
\centering
\caption{\small Ablation Study}
\label{tab:ablation_combined}
\vspace{-1em}
\newcommand{\vhead}[1]{\rotatebox[origin=c]{90}{\textbf{#1}}}
\setlength{\tabcolsep}{3pt} % Tightens internal padding to ensure fit

% Shading definitions
\definecolor{sigdrop}{rgb}{1.0, 0.5, 0.5}
\definecolor{moddrop}{rgb}{1.0, 0.8, 0.8}
\definecolor{slidrop}{rgb}{1.0, 0.9, 0.9}

% --- First Table: Acc@6 ---
\begin{minipage}{0.30\textwidth}
\scriptsize
\centering
\caption*{ (a) Accuracy (Acc@6)}
\vspace{-1.5em}
\begin{tabular}{l|c|ccccc}
\toprule
\textbf{Dataset} & \vhead{\System} & \vhead{w/ Naive $\Preview$} & \vhead{w/ QDMR} & \vhead{w/o Opt. $\mathcal{G}$} & \vhead{w/o Div. $\mathcal{G}$} & \vhead{w/o Pru. $\Schema$} \\ \midrule
\textsf{RepairTQA-S4} & \textbf{0.78} & \cellcolor{moddrop}0.70 & \cellcolor{sigdrop}0.53 & 0.78 & \cellcolor{moddrop}0.66 & \cellcolor{slidrop}0.77 \\ \hline
\textsf{RepairTQA-S3} & \textbf{0.86} & 0.86 & \cellcolor{sigdrop}0.57 & 0.86 & \cellcolor{moddrop}0.79 & \cellcolor{slidrop}0.83 \\ \hline
\textsf{RepairTQA-M1} & \textbf{0.86} & \cellcolor{moddrop}0.78 & \cellcolor{sigdrop}0.37 & 0.86 & \cellcolor{moddrop}0.72 & \cellcolor{slidrop}0.82 \\ 
\bottomrule
\end{tabular}
\end{minipage}% <--- THIS PERCENT IS CRITICAL
\hfill
% --- Second Table: LLM Judge ---
\begin{minipage}{0.30\textwidth}
\scriptsize
\centering
\caption*{ (b) Accuracy (LLM-as-a-Judge)}
\vspace{-1.5em}
\begin{tabular}{l|c|ccccc}
\toprule
\textbf{Dataset} & \vhead{\System} & \vhead{w/ Naive $\Preview$} & \vhead{w/ QDMR} & \vhead{w/o Opt. $\mathcal{G}$} & \vhead{w/o Div. $\mathcal{G}$} & \vhead{w/o Pru. $\Schema$} \\ \midrule
\textsf{RepairTQA-S4} & \textbf{0.65} & \cellcolor{moddrop}0.59 & \cellcolor{sigdrop}0.43 & 0.65 & \cellcolor{moddrop}0.53 & 0.65 \\ \hline
\textsf{RepairTQA-S3} & \textbf{0.74} & 0.74 & \cellcolor{sigdrop}0.46 & 0.74 & \cellcolor{moddrop}0.68 & \cellcolor{slidrop}0.73 \\ \hline
\textsf{RepairTQA-M1} & \textbf{0.70} & \cellcolor{moddrop}0.64 & \cellcolor{sigdrop}0.33 & 0.70 & \cellcolor{moddrop}0.59 & \cellcolor{slidrop}0.68 \\ 
\bottomrule
\end{tabular}
\end{minipage}% <--- THIS PERCENT IS CRITICAL
\hfill
% --- Third Table: Cost ---
\begin{minipage}{0.25\textwidth}
\scriptsize
\centering
\caption*{ (c) Cost}
\vspace{-1.5em}
\begin{tabular}{l|c|c}
\toprule
\textbf{Dataset} & \textbf{\System} & \textbf{w/o Opt. $\mathcal{G}$} \\ \midrule
\textsf{RepairTQA-S4} & \textbf{16.7M} & \cellcolor{moddrop}20.4M \\ \hline
\textsf{RepairTQA-S3} & \textbf{1.3M} & \cellcolor{moddrop}1.6M \\ \hline
\textsf{RepairTQA-M1} & \textbf{0.6M} & \cellcolor{slidrop}0.7M \\ 
\bottomrule
\end{tabular}
\end{minipage}
\vspace{-0.5em}
\end{table*}

==> plots_3.tex <==
\begin{figure*}[!tb] 
\centering
    \includegraphics[width=0.8\textwidth]{figures_arr/legend.pdf}\\
    \begin{minipage}[t]{\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures_arr/dumbbell_representation_comparison.pdf}
        \vspace{-2.0em}
        \caption{\small Robustness comparison of \System vs. baselines on structured vs. semi-structured representation of tables evaluated with \textsc{Gemini-3-Flash}.\nima{double-check all captions.}}
        \label{fig:acc_gemini}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.515\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures_arr/accuracy_combined.pdf}
        \vspace{-2.0em}
        \caption{\small Accuracy comparison of \System vs. baselines.}
        \label{fig:acc_gemini}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.475\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures_arr/cost_combined.pdf}
        \vspace{-2.0em}
        \caption{\small Cost comparison of \System vs. baselines.\protect\footnotemark}
        \label{fig:cost_gemini}
    \end{minipage}
\vspace{-1em}
\end{figure*}


\begin{figure*}[!tb] 
\centering
    \begin{minipage}[t]{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/varying_num_of_plans_accuracy.pdf}
        \vspace{-2.0em}
        \caption{\small Varying no. of plans $K$ vs. accuracy.}
        \label{fig:varying_k_acc}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/varying_batch_size_accuracy.pdf}
        \vspace{-2.0em}
        \caption{\small Varying batch size $\beta$ vs. accuracy.}
        \label{fig:varying_beta_acc}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/varying_num_of_plans_cost.pdf}
        \vspace{-2.0em}
        \caption{\small Varying no. of plans $K$ vs. cost.}
        \label{fig:varying_k_cost}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/varying_batch_size_cost.pdf}
        \vspace{-2.0em}
        \caption{\small Varying batch size $\beta$ vs. cost.}
        \label{fig:varying_beta_cost}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.19\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/error_chart.pdf}
        \vspace{-2.0em}
        \caption{\small Error categorization in \textsf{RepairTQA}.}
        \label{fig:error_analysis}
    \end{minipage}
% \vspace{-1em}
\end{figure*}
\footnotetext{Darker and lighter shades denote \textit{input} and \textit {output} tokens, respectively.}
\begin{table*}[t]
\scriptsize
\centering
\caption{\small Ablation Study}
\label{tab:ablation_combined}
\vspace{-1em}
\newcommand{\vhead}[1]{\rotatebox[origin=c]{90}{\textbf{#1}}}
\setlength{\tabcolsep}{3pt} % Tightens internal padding to ensure fit

% Shading definitions
\definecolor{sigdrop}{rgb}{1.0, 0.5, 0.5}
\definecolor{moddrop}{rgb}{1.0, 0.8, 0.8}
\definecolor{slidrop}{rgb}{1.0, 0.9, 0.9}

% --- First Table: Acc@6 ---
\begin{minipage}{0.30\textwidth}
\centering
\caption*{ (a) Accuracy (Acc@6)}
\vspace{-1.5em}
\begin{tabular}{l|c|ccccc}
\toprule
\textbf{Dataset} & \vhead{\System} & \vhead{w/ Naive $\Preview$} & \vhead{w/ QDMR} & \vhead{w/o Opt. $\mathcal{G}$} & \vhead{w/o Div. $\mathcal{G}$} & \vhead{w/o Pru. $\Schema$} \\ \midrule
\textsf{RepairTQA-S4} & \textbf{0.78} & \cellcolor{moddrop}0.70 & \cellcolor{sigdrop}0.53 & 0.78 & \cellcolor{moddrop}0.66 & \cellcolor{slidrop}0.77 \\ \hline
\textsf{RepairTQA-S3} & \textbf{0.86} & 0.86 & \cellcolor{sigdrop}0.57 & 0.86 & \cellcolor{moddrop}0.79 & \cellcolor{slidrop}0.83 \\ \hline
\textsf{RepairTQA-M1} & \textbf{0.86} & \cellcolor{moddrop}0.78 & \cellcolor{sigdrop}0.37 & 0.86 & \cellcolor{moddrop}0.72 & \cellcolor{slidrop}0.82 \\ 
\bottomrule
\end{tabular}
\end{minipage}% <--- THIS PERCENT IS CRITICAL
\hfill
% --- Second Table: LLM Judge ---
\begin{minipage}{0.30\textwidth}
\centering
\caption*{ (b) Accuracy (LLM-as-a-Judge)}
\vspace{-1.5em}
\begin{tabular}{l|c|ccccc}
\toprule
\textbf{Dataset} & \vhead{\System} & \vhead{w/ Naive $\Preview$} & \vhead{w/ QDMR} & \vhead{w/o Opt. $\mathcal{G}$} & \vhead{w/o Div. $\mathcal{G}$} & \vhead{w/o Pru. $\Schema$} \\ \midrule
\textsf{RepairTQA-S4} & \textbf{0.65} & \cellcolor{moddrop}0.59 & \cellcolor{sigdrop}0.43 & 0.65 & \cellcolor{moddrop}0.53 & 0.65 \\ \hline
\textsf{RepairTQA-S3} & \textbf{0.74} & 0.74 & \cellcolor{sigdrop}0.46 & 0.74 & \cellcolor{moddrop}0.68 & \cellcolor{slidrop}0.73 \\ \hline
\textsf{RepairTQA-M1} & \textbf{0.70} & \cellcolor{moddrop}0.64 & \cellcolor{sigdrop}0.33 & 0.70 & \cellcolor{moddrop}0.59 & \cellcolor{slidrop}0.68 \\ 
\bottomrule
\end{tabular}
\end{minipage}% <--- THIS PERCENT IS CRITICAL
\hfill
% --- Third Table: Cost ---
\begin{minipage}{0.25\textwidth}
\centering
\caption*{ (c) Cost}
\vspace{-1.5em}
\begin{tabular}{l|c|c}
\toprule
\textbf{Dataset} & \textbf{\System} & \textbf{w/o Opt. $\mathcal{G}$} \\ \midrule
\textsf{RepairTQA-S4} & \textbf{16.7M} & \cellcolor{moddrop}20.4M \\ \hline
\textsf{RepairTQA-S3} & \textbf{1.3M} & \cellcolor{moddrop}1.6M \\ \hline
\textsf{RepairTQA-M1} & \textbf{0.6M} & \cellcolor{slidrop}0.7M \\ 
\bottomrule
\end{tabular}
\end{minipage}
\vspace{-0.5em}
\end{table*}
